Bias and Volatility: A Statistical Framework for Evaluating Large Language Model's Stereotypes and the Associated Generation Inconsistency

We present a novel statistical framework for analyzing stereotypes in large language models (LLMs) by systematically estimating the bias and variation in their generation. Current alignment evaluation metrics often overlook stereotypes' randomness caused by LLMs' inconsistent generative behavior. For instance, LLMs may display contradictory stereotypes, such as those related to gender or race, for identical professions in different contexts. Ignoring this inconsistency risks misleading conclusions in alignment assessments and undermines efforts to evaluate the potential of LLMs to perpetuate or amplify social biases and unfairness. To address this, we propose the Bias-Volatility Framework (BVF), which estimates the probability distribution of stereotypes in LLM outputs. By capturing the variation in generative behavior, BVF assesses both the likelihood and degree to which LLM outputs negatively impact vulnerable groups, enabling a quantification of aggregated discrimination risk. Additionally, we introduce a mathematical framework to decompose this risk into bias risk (from the mean of the stereotype distribution) and volatility risk (from its variation). Applying BVF to 12 widely used LLMs, we find: i) Bias risk is the dominant contributor to discrimination; ii) Most LLMs exhibit substantial pro-male stereotypes across nearly all professions; iii) Reinforcement learning from human feedback reduces bias but increases volatility; iv) Discrimination risk correlates with socio-economic factors, such as professional salaries. Finally, we highlight BVF's broader applicability for assessing how generation inconsistencies in LLMs impact behavior beyond stereotypes.

==> Rebuttal/tables/atypical_professions.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{|c|}{Nurse} & \multicolumn{3}{|c|}{Stylist} \\
\cline{2-7}
 & $r$ & $r^p$ & $r^v$ & $r$ & $r^p$ & $r^v$ \\
\hline
Llama2 & 0.2234 & 0.0848 & 0.1386 & 0.3266 & 0.2762 & 0.0504 \\
\hline
GPT2 & 0.3090 & 0.2542 & 0.0548 & 0.3176 & 0.2652 & 0.0524 \\
\hline
BERT & 0.1302 & 0.0896 & 0.0406 & 0.2050 & 0.1916 & 0.0134 \\
\hline
\end{tabular}
\caption{Gender discrimination assessments of atypical professions.}
\label{Atypical}
\end{table}

==> abstract_legacy0217.tex <==
\begin{abstract}
The growing integration of large language models (LLMs) into social operations amplifies their impact on decisions in crucial areas such as economics, education, law, and healthcare,  raising public concerns about these models’ discrimination-related safety and reliability. However, prior discrimination measuring frameworks \textit{solely} assess the average discriminatory behavior of LLMs, often proving inadequate due to the overlook of an additional discrimination-leading factor, i.e., the LLMs' prediction variance across diverse contexts. Moreover, these frameworks commonly rely on crowd-sourced or model-generated test contexts, inevitably introducing biases from humans or other models to the assessment.

In this work, we present the Prejudice-Caprice Framework (PCF) that comprehensively measures discrimination in LLMs by considering both their \textit{consistently biased preference} and \textit{generation randomness} across diverse \textit{automatically generated contexts}. Specifically, we mathematically dissect the aggregated contextualized discrimination risk of LLMs into system risk, originating from LLMs' persistent prejudice, and efficiency risk, stemming from their generation caprice. In addition, we utilize a data-mining approach to gather preference-detecting probes from sentence skeletons, devoid of attribute indications, to approximate LLMs' applied contexts. While initially intended for assessing discrimination in LLMs, our proposed PCF facilitates the measurement of any \textit{inductive biases}, including knowledge alongside prejudice, across \textit{various modality models}.

We apply our discrimination-measuring framework to 12 common LLMs, yielding intriguing findings: \textit{i)} modern LLMs exhibit significant \textit{pro-male stereotypes}, \textit{ii)} LLMs' exhibited discrimination correlates with several social and economic factors, \textit{iii)} system risk dominates the overall discrimination risk and follows a normal distribution, and \textit{iv)} efficiency risk contributes minimally to the overall risk but follows a fat-tailed distribution, suggesting that it is \textit{wild risk} requiring enhanced surveillance.
\end{abstract}
% increasing model size or instruction tuning for alignment with human intents does not guarantee discrimination mitigation

==> conclusion_legacy0218.tex <==
\section{Conclusion}
% We are excited about the future of attention-based models and plan to apply them to other tasks. We plan to extend the Transformer to problems involving input and output modalities other than text and to investigate local, restricted attention mechanisms to efficiently handle large inputs and outputs such as images, audio and video. Making generation less sequential is another research goals of ours.
% Measurement of any inductive biases: X and Y, including knowledge (desired) and prejudice (undesired)

In this study, we propose a Prejudice-Caprice Framework (PCF) to quantify discrimination in LLMs, by considering both their persistent prejudices and preference fluctuations across contexts. Additionally, we enhance the process of gathering test contexts by introducing a data-mining approach designed to avoid introducing human or model biases. Furthermore, our application of the PCF framework to 12 widely utilized models yields valuable insights into the collective stereotypes perpetuated by LLMs, their relationship with societal factors, and the characteristics of their decomposed system and efficiency risks. These findings hold significant implications for discrimination risk management strategies. Finally, we underscore the adaptability of this framework, suggesting its potential for measuring inductive biases across various multimodal models when appropriately tailored.

==> discussions_legacy0218.tex <==
\section{Discussions}
\label{sec:discussions}
While our framework was motivated by discrimination analysis, it is a general framework for measuring and decomposing the model’s behavioral risks. As such, its adaptability enables a wide range of applications, depending on how its components are tailored to specific use cases. In the following sections, we explore the diverse ways in which the framework can be instantiated and deployed across different scenarios.
\subsection{Towards a Unified Framework for Measuring LLM's \textit{Knowledge} and \textit{Prejudice}}
PCF is a statistical framework capable of measuring LLM's \textit{knowledge} and \textit{prejudice}, where the transition between these two measurement scenarios mainly depends on how criterion $J$ is defined. We have mentioned the concept of \textit{inductive biases} several times in previous sections, indicating the conditional relationships among words that the LLM learns from its pre-training data, often inferred from cues like word co-occurrence rates. This represents the LLM's preliminary comprehension of the world gleaned from its exposure to vast textual data. People subjectively label inductive biases that help the LLM accomplish tasks harmlessly as \textit{knowledge}, seen in its ability to generate statements like ``\textit{Pride and Prejudice} is authored by Jane Austen,'' or ``Fubini's theorem states that the order of integration doesn't matter when the integral's absolute value is finite.'' In our work, inductive biases considered as potentially harmful are labeled as \textit{prejudice}, such as when the LLM is more inclined to interpret a demographic group as either victims or criminals, hindering fair judgments, or when it biases a certain group of people towards certain professions, perpetuating social class intergenerational transmission.

Our framework was initially designed to measure this broader notion of \textit{inductive biases}, thus allowing for the assessment of LLM's \textit{knowledge} alongside the \textit{prejudice}. When $J$ is defined to evaluate the LLM's mastery of knowledge, \textit{prejudice} in this work corresponds to \textit{knowledge}, while \textit{caprice} corresponds to \textit{confidence} in this knowledge. More specifically, when $J$ is designed as a concave function of model prediction $p$, according to Jensen's inequality, $\mathbb{E}(J(p)) < J(\mathbb{E}(p))$, indicating that the overall metric $\mathbb{E}(J(p))$ is less than the performance metric of deterministic knowledge $J(\mathbb{E}(p))$ under criterion $J$. The deficit in the overall metric here stems from the \textit{lack of confidence} in knowledge. We leave the refinement of this knowledge measurement framework as future work.

\subsection{\textit{Behavior}: A Comprehensive Evaluation Metrics for Large Foundation Models to Be Grounded in Real-World Applications}
We propose supplementing \textit{performance variance} alongside \textit{average performance} as a holistic measure of the applicability of large foundation models. This entails assessing the overall \textit{behavior} of the model, rather than solely measuring task performance with individual cases. 

Take discrimination measurement, for instance. Human discriminatory viewpoints vary with contexts, influenced by numerous environmental factors during decision-making. For an individual with deep-seated biases yet susceptible to environmental influences, their seemingly fair and benevolent act in a particular context requires explanation using both the mean and variance of their biased \textit{preferences}. For LLMs, instances where the generation distribution shifts due to varied conditioned contexts are more readily observable. For example, inconsistencies in LLM predictions on case judgments due to subtle changes in wording that do not affect the facts of the case pose a serious threat to judicial fairness \citep{chen2023knowledge}. Hence, in considering the model's application risks, both \textit{prejudice} and \textit{caprice across contexts} need to be taken into account. 

The same rationale applies to measuring LLM knowledge. Inconsistency in model knowledge generation, indicative of insufficient knowledge confidence, also impacts the model's application effectiveness. 

Hence, we suggest that in model auditing, in addition to the traditional measure of \textit{average task performance}, one should also take into account \textit{performance variance}, indicating inconsistencies in behavior across various contexts. Indeed, much akin to evaluating human performance across diverse situations when recruiting labor, we should similarly assess the holistic \textit{behavior} of models before deploying them in real-world applications.

\subsection{Expanding the Scope of \textit{Context} to Evaluate Inductive Biases Across Modalities}
Expanding the scope of \textit{context} allows this framework to measure the inductive bias of models across diverse modalities. In this study, context primarily refers to the textual environment upon which the LLM is conditioned, while for visual models, such as those in autonomous vehicles determining steering angles from visual inputs, the context covers all encountered visual scenarios. 

Evaluating the inductive biases of models across modalities is equally essential for their safe practical deployment. For instance, assessing the qualification of a visual model for autonomous vehicles requires at least measuring its knowledge of traffic-norm related video-action pairs such as \textit{<video: running emergency vehicle, action: yield>}, where the videos constitute the major contexts. In testing this knowledge, visual contexts should encompass not only commonly encountered emergency vehicles like ambulances and police cars but also ones from the long-tail distribution, such as fire trucks \citep{autonomous-driving-fire-truck}. Likewise, determining the applicability of this visual model for autonomous driving systems also necessitates the evaluation of both the average performance and the performance variance regarding a set of traffic knowledge of a similar nature.

==> format.tex <==
\section{Submission of papers to NeurIPS 2023}


Please read the instructions below carefully and follow them faithfully. \textbf{Important:} This year the checklist will be submitted separately from the main paper in OpenReview, please review it well ahead of the submission deadline: \url{https://neurips.cc/public/guides/PaperChecklist}.


\subsection{Style}


Papers to be submitted to NeurIPS 2023 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.


The margins in 2023 are the same as those in previous years.


Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.


\subsection{Retrieval of style files}


The style files for NeurIPS and other conference information are available on
the website at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2023.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.


The only supported style file for NeurIPS 2023 is \verb+neurips_2023.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}


The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.


\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit, as long as you do not say which conference it was submitted to. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS. 


At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.


The file \verb+neurips_2023.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.


The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.


\section{General formatting instructions}
\label{gen_inst}


The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.


The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.


For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.


Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.


\section{Headings: first level}
\label{headings}


All headings should be lower case (except for first word and proper nouns),
flush left, and bold.


First-level headings should be in 12-point type.


\subsection{Headings: second level}


Second-level headings should be in 10-point type.


\subsubsection{Headings: third level}


Third-level headings should be in 10-point type.


\paragraph{Paragraphs}


There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.


\section{Citations, figures, tables, references}
\label{others}


These instructions apply to everyone.


\subsection{Citations within the text}


The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.


The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}


If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2023+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}


If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2023}
\end{verbatim}


As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous'' and include a copy of the anonymized paper in the supplementary material.


\subsection{Footnotes}


Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).


Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}


\subsection{Figures}


\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}


All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.


You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.


\subsection{Tables}


All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.


Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.


Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.


\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Math}
Note that display math in bare TeX commands will not create correct line numbers for submission. Please use LaTeX (or AMSTeX) commands for unnumbered display math. (You really shouldn't be using \$\$ anyway; see \url{https://tex.stackexchange.com/questions/503/why-is-preferable-to} and \url{https://tex.stackexchange.com/questions/40492/what-are-the-differences-between-align-equation-and-displaymath} for more information.)

\subsection{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.


\section{Preparing PDF files}


Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''


Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.


\begin{itemize}


\item You should directly generate PDF files using \verb+pdflatex+.


\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.


\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.


\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


\end{itemize}


If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.


\subsection{Margins in \LaTeX{}}


Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})


A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.


\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2023/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}



\section{Supplementary Material}

Authors may wish to optionally include extra information (complete proofs, additional experiments and plots) in the appendix. All such materials should be part of the supplemental material (submitted separately) and should NOT be included in the main submission.


\section*{References}


References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip

\bibliography{neurips_2023}
\bibliographystyle{unsrt}

\iffalse
{
\small


[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.


[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.


[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
}
\fi

==> formula.tex <==
\section{formula}
The vectorial representation of the stereotypical direction associated with a particular group, denoted as $g \in G$, is characterized by a multi-dimensional vector of length $|G|$. This can be mathematically expressed as follows:
\begin{equation}
    d_{g} = \left( -\frac{1}{|G|-1}, -\frac{1}{|G|-1}, \ldots, 1, \ldots, -\frac{1}{|G|-1} \right),
\end{equation}
wherein the $g^{th}$ element is designated as 1, whilst the remaining elements are uniformly assigned the value $-\frac{1}{|G|-1}$.

Discrimination Level Criterion $J_{g}$ describes the degree of overlap between model prediction and the stereotype:
\begin{equation}
    J_{g}(p)=max\{<p, d_{g}>, 0\}
\end{equation}
where $<p, d_{g}>$ is the inner product of probability distribution prediction $p$ and discriminatory direction $d_g$.

The Overall Discrimination Risk $R$:
\begin{equation}
    R = \mathbb{E}_X\max_{g}\mathbb{E}_T (J_g(p_{X,T}))
\end{equation}
The Overall System Risk:
\begin{equation}
    R_s = \mathbb{E}_X\max_{g} J_g(\mathbb{E}_T(p_{X,T}))
\end{equation}
The Overall random Risk:
\begin{equation}
    R_r = \mathbb{E}_X\max_{g} [\mathbb{E}_T (J_g(p_{X,T}))- J_g(\mathbb{E}_T(p_{X,T}))]
\end{equation}
\textcolor{red}{Would it be better to replace $\max_{g}$ with $\mathbb{E}_{g}$?}

==> implementation_details_with_context_template_mining_approach.tex <==
%\section{Implementation Details with Context Template Mining Approach}
\label{sec:implementation_details_with_context_template_mining_approach}

In this section, we elucidate how to implement our discrimination-measuring framework, outlined in Section \ref{sec:mathematical_modeling_of_social_discrimination_and_risk_decomposition}, using real-world data. The primary consideration is selecting the appropriate context format based on the model type being assessed. For instance, for language models, context means textual environments, while for image classifiers, it entails the set of images awaiting classification. Simply put, the context serves as the backdrop for model predictions, providing supporting evidence while adapting to the model’s training and application paradigms to optimally invoke the model's inductive bias. In our experiments, we focus on evaluating LLMs, thus using textual contexts. While we automated context template extraction with a data mining approach, determining whether to incorporate human prior knowledge or AI-human collaborative intelligence when defining context to best replicate the distribution of the model’s real-world applications, are intriguing questions left for future exploration. As an example, we consider $X$ as \textit{occupations} and $Y$ as \textit{binary gender}\footnote{We acknowledge diverse gender identities and employ a binary framework only for experimental consistency with prior research.}.

\subsection{Define $X$ and $Y$}
$X$ comprises gender-neutral occupation terms, and their corresponding probability distribution that serve as aggregation weights for calculating discrimination risk. The occupation list used is provided in Appendix \ref{app:X}. The distribution of these terms indicates the emphasis placed on each occupation when assessing the application risk of LLMs. We utilize two distribution sets: (i) a uniform distribution without occupation value judgments, and (ii) demographical statistics from official labor statistics sources \citep{employment-by-detailed-occupation}, assigning weights based on the number of individuals in each industry. Details on the latter are provided in Appendix \ref{app:J}.

$Y$ consists of groups of gender-specific terms shaping societal perceptions of each gender, with each term having a counterpart in every other group. For instance, $Y$ typically comprises two sub-groups: $Y_{masculine}$ and $Y_{feminine}$. The former includes words such as \textit{he}, \textit{man}, \textit{grandfather}, etc., while the latter consists of corresponding words like \textit{she}, \textit{woman}, \textit{grandmother}, etc. Word lists for $Y$ employed in this work are available in Appendix \ref{app:Y}.

\input{Figures/template_mining}

\subsection{Collect $T$ with a Data Mining Approach}
$T$ stands for a set of context probes meticulously collected to unveil the preferences of LLMs, with its distribution recorded to approximate the operational context of LLMs. These context templates are specifically devised to link $X$ and $Y$. Consequently, when the template is enriched with a term from $X$, and the LLM engages in contextual inference, its prediction of the next or masked tokens can mirror its stance toward the topic $Y$.

To mitigate the biases from humans or other models that would contradict the goal of measuring biases impartially, we employ a data mining approach for collecting context templates. Given the potential presence of gender-indicative adjectives or adverbs in complex sentence structures, we selectively retain the skeletal structures, i.e. the essential structural elements of a sentence, often represented by the main phrases or clauses that convey the primary meaning, and tally their occurrences. The acquisition of $T$ follows the outlined steps (also depicted in Figure \ref{fig:template_mining}).

\paragraph{Step 1. Gather sentences containing terms from $Y$ to create $T^{Elementary}$.}
We randomly sample 10,000 articles from Wikipedia for our mining dataset. In preprocessing the data, we filter out sentences lacking words from $Y$\footnote{Ideally, we'd focus on sentences with terms from both $X$ and $Y$. Yet, in practice, we found these sentences to be scarce, hindering corpus construction. As a result, we ease this constraint.}. Next, we retain only those sentences where the gender-specific word from $Y$ either co-refers with or modifies the subject. The structural skeletons of these selected sentences offer additional contextual cues to LLMs, encouraging them to express nuanced attitudes towards $Y$ during inference.

\paragraph{Step 2: Utilize syntax analysis tools to extract syntactic patterns from sentences in $T^{Elementary}$.}
We simplify intricate text structures into sentence skeletons, reducing gender-specific cues for LLMs' inference, and then we track these predicates' frequency, marked by $Count(\cdot)$. For instance, in the sentence ``\textcolor{MALE_COLOR}{Detective Smith} said \textcolor{MALE_COLOR}{he} would leave no stone unturned...'' where \textcolor{MALE_COLOR}{\textit{he}} refers to \textcolor{MALE_COLOR}{\textit{Detective Smith}} and belongs to $Y_{masculine}$, we parse and extract the predicate situated between these keywords, simply \textit{said} here, without imposing restrictions on its length. All predicates are standardized to the past tense, and \textit{that} is appended to reporting verbs, to prevent counting predicates with equivalent meanings, such as \textit{says}, \textit{said}, and \textit{said that}, multiple times. Context templates are crafted using ``[X]'' for the subject and ``[Y]'' for the gender attribute word, as in ``\textcolor{TEMPLATE_COLOR}{The [X] said that [Y]}.'' We assume minimal deviation between the distribution of the mining dataset and real-world LLM application contexts. Consequently, the weight of each context template for aggregation is determined by its frequency in the mining dataset, calculated as $\frac{Count(t_i)}{\sum_{t \in T} Count(t)}$. Detailed information about our chosen $T$ and its distribution is available in Appendix \ref{app:T}.

\subsection{Apply Real-world Data to Our Framework}
As specified in Equation \ref{eq:d_y} and with $|Y|=2$ in our experimental setup, we assign $\mathbf{d}_{masculine}$ as $(1, -1)$ and $\mathbf{d}_{feminine}$ as $(-1, 1)$.

$\mathbf{p}_{t, x}$ denotes the gender-relevant probability distribution generated by the PLM $M_{\Theta}$ when provided with the context template $t$ and substituting ``[X]'' with the occupation $x$:

\begin{align}\label{eq:pij}
    \mathbf{p}_{t, x}=[\frac{\sum_{y\in Y_u}\hat{\mathbf{p}}_{t, x}(y)}{\sum_{y\in \cup\{Y_u\}}\hat{\mathbf{p}}_{t, x}(g)}, u\in \{1, \ldots, |Y|\}]\\
    where\quad\hat{\mathbf{p}}_{t, x}(\cdot)=M_{\Theta}(t, x)[index(\cdot)]
\end{align}

where we calibrate the models' preferences so that the numerator aggregates all probabilities associated with a set of gender words, while the denominator acts as the normalization factor.

With $\mathbf{d}_y$ and $\mathbf{p}_{t, x}$ defined, along with Equations \ref{eq:J} to \ref{eq:R^p}, we can apply our datasets $X$ (with distribution), $Y$, and $T$ (with distribution) to compute $r_x, r_x^p, r_x^c$ and their correpsonding $R, R^p, R^c$.

==> intro_old.tex <==
\section{Introduction}
\input{Figures/intuitive_understanding}
The penetration of large language models (LLMs) into society heightens public apprehension regarding the potential for its algorithmic bias to induce or exacerbate social inequality \citep{barocas2017problem,cowgill2018bias,deshpande2020mitigating,dressel2018accuracy,Reuters2018Amazon}. For instance, job matching systems powered by LLMs could unintentionally disadvantage ethnic minorities or individuals with disabilities \citep{hutchinson2020social}. Similarly, modern machine translation systems often transform gender-neutral terms into predominantly gendered forms, potentially intensifying existing gender biases  \citep{stanovsky-etal-2019-evaluating}. Consequently, there is an urgent call for effective metrics to assess these detrimental biases in LLMs, ensuring their fair applications.

As the generation of LLMs fluctuates unpredictably in response to subtle changes in the given prompts \citep{li2023nuances,li2024mutation} with illustration in Figure \ref{fig:intuitive_understanding} and Figure \ref{fig:heatmap}, the stereotypes associated with a justice-related topic demonstrated by an LLM should be conceptualized as random vectors to model the uncertainty. \cheng{Figure 1 shows decomposition of two types of errors, but here they aren't explained. How about moving the discussion of Figure 1 to a point after we introduce the framework? This second paragraph only needs to point out the limitations of the existing work, which would then be followed immediately by the third paragraph where we'll say we propose a new framework to address the limitations. } For instance, an LLM's binary gender stereotype regarding a profession can be represented as a two-dimensional random variable, where each dimension corresponds to the probability of the profession being male/female. Here, the randomness stems from the LLMs' fragility to the slight variations in the contexts. Therefore, it necessitates identifying statistical patterns in the model's stereotype, including considering statistics (mean, distribution etc.) of the behavioral metrics across diverse contexts. \cheng{Is the consideration of the whole distribution a novel aspect of our paper or is it something already suggested in any existing work? If it's a novel idea in our paper, I think we should move this discussion after we say we introduce a new framework, where we'd then say the key idea is to attempt to characterize the whole distribution more completely than existing work.} Though such randomness will lead to severe societal consequences \citep{dahan2023lawyers,nastasi2023vignette,chougule2023comprehensive}, previous assessments have predominantly focused on measuring LLMs' normal discriminatory behaviors \citep{nadeem2020stereoset,nangia2020crows}. In other words, they only criticize the model for ``typically making a particular biased inference,'' overlooking the potential discrimination risks triggered by the LLMs' generation inconsistency and unpredictability. \cheng{this criticism is vague and too generic. Can we make it clearer? As is, it's unclear how the proposed new framework mentioned in the next paragraph would be better. A general comment here is that the novelty of our work isn't articulated explicitly with a direct connection to deficiency of previous work. Also, an analysis of the cause of deficiency of previous work would help. E.g., it was caused by not viewing the LLM as a stochastic random variable(?) or otherwise, we can say in order to achieve the goal ..., we must model the prediction of an LLM as a random variable, i.e., a Bayesian view, which would then allow us to quantify the variance, not just capturing the mean.... }

 % As LLMs' generation fluctuate unpredictably in response to subtle changes in the given prompts (as depicted in Appendix Figure \ref{fig:intuitive_understanding} and examples), it necessitates identifying statistical patterns in the model's behavior, including considering statistics (mean, variance, quantile etc.) of the LLM behavior metrics under diverse contexts. However, previous assessments have predominantly focused on LLMs' normal discriminatory behaviors \citep{nadeem2020stereoset,nangia2020crows}. In other words, they only criticize the model for ``typically making a particular biased inference,'' overlooking the potential discrimination risks triggered by the LLMs' generation inconsistency and unpredictability. 

% \ke{Nightmare starts here.} 
% Therefore, assessing the discrimination risk of LLM integration necessitates estimating the LLM's stereotype distribution and establishing comprehensive metrics based on this distribution to quantify the magnitude of the discrimination risk. For example, a language model that always asserts a doctor to be male in half of the contexts and female in the other half poses a greater risk of bias than a language model that indicates an equal likelihood of being male or female in all contexts. \ke{Not necessarily?} This is because the former carries risks to propagate new stereotypes or reinforce existing ones. \ke{From a reader's perspective, it's an unsuccessful example, failing to exemplify anything.} As LLMs' generation fluctuate unpredictably in response to subtle changes in the given prompts (as depicted in Appendix Figure \ref{fig:intuitive_understanding} and examples), 




% However, the method of estimating LLMs' stereotype distribution is absent and difficult to develop. Previous assessments have predominantly focused on LLMs' normal discriminatory behaviors \citep{nadeem2020stereoset,nangia2020crows}. Their method is distinct from estimating the stereotype distribution of LLMs, which is challenging. LLM's stereotype distribution has not been rigorously defined in mathematical terms. The set of contexts that may lead to stereotype generation by LLMs has not yet been defined or studied. Meanwhile, estimating LLM's stereotype distribution involves computational complexity. For instance, it is hard to figure out all gender-discrimination-related contexts from all contexts. 

In this work, we propose the Prejudice-Volatility Framework (PVF) that introduces statistical metrics for characterizing the LLMs' stereotype probability distribution, and accordingly evaluates the risk of discrimination in LLM applications. To elaborate, we initially establish a mathematical definition for the \textit{LLM's stereotype distribution} based on their token prediction probabilities. Furthermore, we employ a data-mining approach to approximate the LLMs' applied contexts, enabling the estimation of the stereotype distribution. Subsequently, we propose metrics to assess and compare biased behavioral patterns in LLMs, while also dissect the origins of discrimination with theoretical substantiation. In contrast to existing bias assessment frameworks, our approach offers several distinguishing features: \textit{i)} Versatility: Our framework can be adapted for diverse measurement objectives concerning justice- or fairness-related topics; \textit{ii)} Comparative analysis: It enables the comparison of discrimination risk across different LLMs; and \textit{iii)} Causative analysis: Our method provides a clear delineation of the sources of discrimination, elucidating whether it stems from the model's learned biases or its generation inconsistency. Originally designed for measuring LLMs' discrimination, our proposed PVF allows statistical analysis and comparison of parametric biases, i.e. knowledge and prejudice, in any modal model, provided the framework's components are appropriately adapted for that use case (refer to Appendix \ref{sec:discussions} for more details).

% We developed the Prejudice-Volatility Framework (PVF) for estimating LLM's stereotype distribution function and assessing the discrimination risk level induced by LLM's penetration. According to the concept of the probability of tokens, our study mathematically defined LLM's stereotype distribution. Our definition enables us to apply the data-mining approach to approximate the possible applied contexts of LLMs leading to potential stereotypes and estimate the stereotype distribution function. We further developed a protocol to generate the metric for assessing and comparing LLM-induced social injustice risk levels. Compared with the bias measurements in the literature, our method has the following advantages: First, our method can calculate the probability of LLMs' stereotypes for any specific justice and fairness topics. Second, our method allows the comparison between different LLMs for various tasks. Third, our method allows the analysis of whether an LLM's stereotype is caused by the model's systematic bias. We thus develop a method to decompose the contribution of LLM's system bias on stereotypes from that of LLM's other statistical features. The decomposition reveals how much an LLM's stereotype is due to its systematic prejudice or statistical volatility.


We apply our evaluation framework to 12 commonly used language models, providing insights and issuing pre-warnings on the risk of employing potentially biased LLMs. Key points include:  \textit{i)} Prejudice risk dominates the overall assessed discrimination risk, implying that the system bias in LLMs is the root cause of model stereotype; \textit{ii)} Most LLMs demonstrate significant pro-male stereotypes across nearly all careers; \textit{iii)} LLMs that undergo alignment with Reinforcement Learning from Human Feedback exhibit a lower overall discrimination risk, attributed to decreased prejudice risk, yet they showcase higher volatility risk; \textit{iv)} LLMs' discrimination risk correlates with crucial social and economic factors such as profession salary.

==> introduction_copy.tex <==
\section{Introduction}



The penetration of large language models (LLMs) into society heightened public apprehension regarding the potential for its algorithmic bias to induce or exacerbate social inequality \citep{barocas2017problem,cowgill2018bias,deshpande2020mitigating,dressel2018accuracy,Reuters2018Amazon}. For instance, job matching systems powered by LLMs could unintentionally disadvantage ethnic minorities or individuals with disabilities \citep{hutchinson2020social}. Similarly, modern machine translation systems often transform gender-neutral terms into predominantly gendered forms, potentially intensifying existing gender biases  \citep{stanovsky-etal-2019-evaluating}. Consequently, there is an urgent call for effective mechanisms to assess these detrimental biases in LLMs, ensuring their fair applications.

As LLMs' generation fluctuate unpredictably in response to subtle changes in the given prompts (as depicted in Appendix Figure \ref{fig:intuitive_understanding} and examples), it necessitates identifying statistical patterns in the model's behavior, including considering statistics (mean, variance, quantile etc.) of the LLM behavior metrics under diverse contexts. However, previous assessments have predominantly focused on LLMs' normal discriminatory behaviors \citep{nadeem2020stereoset,nangia2020crows}. In other words, they only criticize the model for ``typically making a particular biased inference,'' overlooking the potential discrimination risks triggered by the LLMs' generation inconsistency and unpredictability. This lack of attention to model prediction variations prevents accurate evaluation of biased LLMs in the following scenarios:

\textit{Suppose the unbiased preference is $\mathbf{p}^\star=(\textcolor{MALE_COLOR}{0.5}, \textcolor{FEMALE_COLOR}{0.5})$. We have two models, $M_1$ and $M_2$, each displaying preferences in contexts $\{C_1, C_2, C_3\}$, with the corresponding system biases and preference errors computed as follows: }

\begin{center}
    $M_1: \{C_1: (\textcolor{MALE_COLOR}{0.6}, \textcolor{FEMALE_COLOR}{0.4}), C_2: (\textcolor{MALE_COLOR}{0.6}, \textcolor{FEMALE_COLOR}{0.4}), C_3: (\textcolor{MALE_COLOR}{0.6}, \textcolor{FEMALE_COLOR}{0.4})\}, system~bias=\textcolor{RISK_COLOR}{\textbf{0.1}}, error=\textcolor{RISK_COLOR}{\textbf{20\%}}$;
\end{center}

\begin{center}
    $M_2: \{C_1: (\textcolor{MALE_COLOR}{0.5}, \textcolor{FEMALE_COLOR}{0.5}), C_2: (\textcolor{MALE_COLOR}{0.35}, \textcolor{FEMALE_COLOR}{0.65}), C_3: (\textcolor{MALE_COLOR}{0.65}, \textcolor{FEMALE_COLOR}{0.35})\}, system~bias=\textcolor{RISK_COLOR}{\textbf{0}}, error=\textcolor{RISK_COLOR}{\textbf{20\%}}$.
\end{center}

\textit{where the system bias quantifies the difference between a model's average contextualized preferences and the unbiased preference. }

In this case, both LLM discrimination metrics (\textit{system bias} and \textit{error}) erase crucial contextual details. Firstly, system bias overlooks the variation of the model's preferences, which reflects inconsistency in their predictions or decision-making, as seen in the case of $M_2$. $M_2$ exhibits biased preferences in most contexts, yet its system bias remains at $\textcolor{RISK_COLOR}{\textbf{0}}$. Furthermore, error alone fails to capture the drastic attitude shift of the model. For instance, comparing $M_1$ and $M_2$, while both have the same error to be $\textcolor{RISK_COLOR}{\textbf{20\%}}$, it does not account for $M_2$'s context-dependent preference changes, which are even more pronounced in some situations. Consequently, a comprehensive quantitative measure of model discrimination should \textit{i)} consider both \textit{average performance} and \textit{performance variation}, termed \textit{prejudice} and \textit{caprice} in our study, respectively; and \textit{ii)} facilitate their decomposition accordingly.

\input{Figures/framework}

% implying the language model beneath is a unigram model
As illustrated in Figure \ref{fig:framework}, we hereby introduce a Prejudice-Caprice Framework (PCF) to comprehensively measure social discrimination in LLMs, by considering not only the models’ \textit{consistent discriminatory performance} but also their \textit{performance variation across multiple contexts}. Practically speaking, we investigate the inductive bias of LLMs towards a demographical group $Y$ given another demographical group $X$ as the evidence. This exploration involves statistically analyzing LLMs' predicted word probabilities conditioned on context templates augmented with $X$, whose distribution aligns with that of the applied contexts of LLMs. It is noteworthy that $X$ and $Y$ could be instantiated for various measurement objectives, for example, $X$ as \textit{occupations} and $Y$ as \textit{gender} for assessing discrimination within each industry, or $X$ as \textit{education year} and $Y$ as \textit{income} for evaluating the impact of education on social stratification. In addition, we provide the mathematical decomposition of our proposed discrimination risk into \textit{prejudice} risk and \textit{caprice} risk. PCF exhibits the following properties: \textit{i)} an ideally unbiased model has an overall discrimination risk of 0, \textit{ii)} a stereotyped model has the highest prejudice risk and 0 caprice risk, and \textit{iii)} a randomly stereotyped model shows 0 prejudice risk but the highest caprice risk\footnote{Originally designed for measuring LLMs' discrimination, our proposed PCF allows statistical analysis and comparison of inductive biases, i.e. knowledge and prejudice, in any modal model, provided the framework's components are appropriately adapted for that use case (refer to Section \ref{sec:discussions} for more details).}. 

We also introduce a data-mining approach to collecting templates that can approximate the applied context of LLMs. We avoid crowd-sourced or LLM-generated context templates to prevent introducing prior biases from humans or other models. Therefore, our framework serves as an exhaustive audit for evaluating social discrimination in LLMs, contributing to the communities’ collective efforts to develop transparent, fair, and reliable models.

We apply our evaluation framework to 12 widely used language models, providing insights and issuing pre-warnings on the risk of employing potentially biased LLMs. Key points include: \textit{i)} all our examined models exhibit notable \textit{pro-male} bias, \textit{ii)} LLMs’ \textit{prejudice} contributes significantly to the application risk of larger models, and shows strong correlations with social and economic factors such as salary and education year, and \textit{iii)} the risk from LLMs’ \textit{caprice} follows a fat-tailed distribution, indicating a hard-to-predict \textit{wild risk} defying the law of large numbers, which requires strengthened surveillance and regulatory measures.

% \textit{ii)} increasing the model size and incorporating human feedback in LLMs’ training doesn’t guarantee improved fairness, \textit{iii)} LLMs’ \textit{prejudice} contributes significantly to the application risk of larger models, and shows strong correlations with social and economic factors such as salary and education year, and \textit{iv)} the risk from LLMs’ \textit{caprice} follows a fat-tailed distribution, indicating a hard-to-predict \textit{wild risk} defying the law of large numbers, which requires strengthened surveillance and regulatory measures.

==> introduction_legacy0207.tex <==
\section{Introduction}
\input{Figures/intuitive_understanding}
% Large Language Models (LLMs), harnessing insights from extensive real-world datasets, exhibit remarkable proficiency in text generation. \ke{Some proficient paper writers suggest that I should start my writing with a sentence which not only introduces the pertinent background but also reveals the theme or purpose of the paper, which also applies here.} \ke{My attempt: Large Language Models (LLMs) of today, while exhibiting impressive world prior knowledge after being pre-trained on web-scaled data, pose risk when they are applied to real-world tasks, as they may inadvertently perpetuate or amplify existing prejudices present in the training data, potentially leading to unfair and even detrimental outcomes towards specific individuals or groups.} Yet, in numerous instances, these models are publicly concerned to operate detrimentally towards specific individuals or groups. For example, employment matching systems might inadvertently impose disadvantages upon minority ethnicities or individuals with disabilities (Hutchinson et al., 2020) \ke{\textbackslash citep here?}. Similarly, machine translation systems often convert gender-neutral terms into predominantly gendered forms, thereby potentially amplifying pre-existing gender biases (Stanovsky et al., 2019). Furthermore, these models may engender discriminatory outcomes in crucial sectors such as credit authorization, judicial decision-making, and healthcare, \ke{Consequently, the occasional biased generation of LLMs might have adverse effects on critical decisions, such as those related to credit authorization, judicial decision-making, and healthcare,} which not only infringes upon individual rights but also erodes the fundamental principles of equality (Barocas and Selbst, 2016). More broadly, the biases and misinformation disseminated by generative models could significantly distort societal perceptions in hitherto unforeseen manners (Kidd and Birhane, 2023) \ke{What do you mean by "unforeseen manners?"}. %(unprecedented ways)

While large language models (LLMs) exhibit impressive world prior knowledge after being pre-trained on web-scaled data, they pose risks when applied to real-world tasks, as their generation may inadvertently perpetuate or amplify existing social discrimination present in the training data, potentially leading to unfair and even detrimental outcomes towards specific individuals or groups \citep{bolukbasi2016man,sheng2020nice,mei2023bias}. For instance, job matching systems powered by LLMs could unintentionally disadvantage ethnic minorities or individuals with disabilities \citep{hutchinson2020social}. Similarly, modern machine translation systems often transform gender-neutral terms into predominantly gendered forms, potentially intensifying existing gender biases  \citep{stanovsky-etal-2019-evaluating}. Consequently, the biased generation of LLMs might have adverse effects on critical decisions, such as those related to credit authorization, judicial decision-making, and healthcare, endangering individual rights and the fundamental principles of equality \citep{barocas2017problem,cowgill2018bias,deshpande2020mitigating,dressel2018accuracy,Reuters2018Amazon}. 

% \ke{Large Language Models (LLMs) of today, while exhibiting impressive world prior knowledge after being pre-trained on web-scaled data, pose risk when they are applied to real-world tasks, as they may inadvertently perpetuate or amplify existing prejudices present in the training data, potentially leading to unfair and even detrimental outcomes towards specific individuals or groups. For instance, job matching systems powered by LLMs could unintentionally disadvantage minority ethnicities or individuals with disabilities \citep{}. Similarly, modern machine translation systems often transform gender-neutral terms into predominantly gendered forms, potentially intensifying existing gender biases \citep{}. Consequently, the biased generation of LLMs might have adverse effects on critical decisions, such as those related to credit authorization, judicial decision-making, and healthcare, not only infringing upon individual rights, but also eroding the fundamental principles of equality \citep{}.}
As depicted in Figure \ref{fig:intuitive_understanding}, given the fluctuation in the potentially biased generation of LLMs across \textit{applied contexts\footnote{In the case of LLMs, \textit{contexts} refer to their textual operational settings, such as varied job requirements and candidate resumes for job matching, or diverse case keywords and legal databases for legal information retrieval.}}, measuring social discrimination in LLMs, much akin to assessing it in humans, requires ample samples to uncover their underlying bias patterns.  As LLMs typically follow a language modeling paradigm throughout training and usage, they demonstrate \textit{preferences} by conditioned word probability prediction. Specifically, whether generating evaluation reports from job applicants' resumes \citep{gan2024application} or extracting legal information for judicial decisions \citep{wu2023precedent}, these models essentially develop responses implying their inductive biases by calculating and maximizing the probability of the next (or masked) tokens highly dependent on scenario-specific contexts. Therefore, evaluating the LLMs’ discrimination and application risk necessitates restoring their use cases because LLMs act as probability estimators for desired tokens conditioned on their deployment contexts. The statistical properties of their predicted distributions, such as persistent preferences for certain demographical groups, faithfully reflect their learned biases when supplemented with conditions, i.e. contexts, that closely resemble their operational environments.
% While large language models (LLMs) exhibit impressive world prior knowledge after being pre-trained on web-scaled data, they pose risks when applied to real-world tasks, as their generation may inadvertently perpetuate or amplify existing social discrimination present in the training data, potentially leading to unfair and even detrimental outcomes towards specific individuals or groups \citep{bolukbasi2016man,sheng2020nice,mei2023bias}. For instance, job matching systems powered by LLMs could unintentionally disadvantage ethnic minorities or individuals with disabilities \citep{hutchinson2020social}. Similarly, modern machine translation systems often transform gender-neutral terms into predominantly gendered forms, potentially intensifying existing gender biases  \citep{stanovsky-etal-2019-evaluating}. Consequently, the biased generation of LLMs might have adverse effects on critical decisions, such as those related to credit authorization, judicial decision-making, and healthcare, endangering individual rights and the fundamental principles of equality \citep{barocas2017problem,cowgill2018bias,deshpande2020mitigating,dressel2018accuracy,Reuters2018Amazon}. 

% However, quantifying the discriminatory risks posed by language models in practical applications poses substantial challenges. Firstly, the responses generated by language models can vary for identical or similar queries, even when the query formulation remains consistent (Jang et al., 2021). In contrast to human bias scales, where a limited set of test questions can yield statistically relevant findings, thoroughly auditing a model necessitates a more granular array of test data to accurately assess discrimination risks. Secondly, most existing research on LLM bias necessitates predefined phrases or stereotypes linked to bias. These stereotypes are challenging to exhaustively identify, as they are subject to constant evolution and change. Moreover, the biases identified are often reflective of those prevalent in human societies, neglecting the possibility that LLMs might generate biases that exceed human expectations. Lastly, the application of language models across diverse linguistic contexts entails varying bias risk scenarios. Current bias measurement datasets may be ill-equipped to address all different language scenarios. 
%\ke{Here, I personally believe we should emphasize that this is an exhaustive framework, i.e., explaining \textbf{where algorithmic auditing should be} and thereafter why we could claim our proposed framework end the ``algorithmic auditing'' problem. What any following studies could do is only to improve this method by adjusting its components.} \ke{My such belief comes from several facts: i) When we are auditing LLMs, we are essentially measuring whether some of their parametric prior knowledge are ``biased'' (it's note-worthy that the defintion of bias varies among different groups of people); considering the universal and consistent language modeling objective in the LLMs' training and testing paradigm, we have to reconstruct the LLMs' application scenarios (the conditioned contexts) in order to measure their risk. ii) Discrimination risk is exclusively determined by the static/general system's prejudice and the specific context its generation is conditioned on (a.k.a. caprice), and the cost or risk of loss for these two elements varies depending on the application scenarios, like medical vs. legal and judicial, so it's necessary for the auditing framework to spilt them apart.} \ke{The logic would be: i) auditing LLMs requires extensive contexts, so we automate context generation, ii) auditing LLMs requires risk decomposition, so we figure out how to decompose it.} \ke{Of course, enumerating the drawbacks of previous work matters. But if we shift our tone to ``we device our framework based on our understanding of what algorithmic auditing of LLMs should look like instead of trying to supplement previous work'', the writing would be more appealing.}

% To assess the social discrimination in LLMs and the empirical risk of employing these models in specific scenarios, it's essential to reconstruct their \textit{application contexts}. Modern LLMs typically follow a universal language modeling paradigm throughout both training and usage. Specifically, whether generating evaluation reports from job applicants' resumes \citep{gan2024application} or extracting legal information for judicial decisions \citep{wu2023precedent}, these models essentially develop responses by calculating and maximizing the probability of the next (or masked) tokens highly dependent on scenario-specific contexts. Therefore, evaluating the LLMs’ discrimination and application risk necessitates restoring their use cases because LLMs act as probability estimators for desired tokens conditioned on their deployment contexts. The statistical properties of their predicted distributions, such as persistent preferences for certain demographical groups, faithfully reflect their learned biases when supplemented with conditions, i.e. contexts, that closely resemble their operational environments.

Moreover, as the application risk of biased LLMs is closely tied to the parametric biases acquired during their pre-training, and the inconsistency and unpredictability in their generated responses to varied but subtly different contexts, with distinct harm severity associated with these two risk sources, a prudent risk measurement framework should systematically dissect the risk into these components, in our work termed as \textit{prejudice} and \textit{caprice}, respectively. Such a risk decomposition step will significantly improve our understanding and effective management of the overall risk.

% Language models serve as estimators of conditional probabilities for specific input texts, wherein their statistical outputs regarding the unfairness of these probabilities towards protected groups indicate the magnitude of discrimination risk. In light of the consistent and universal objectives of language modeling in the training and testing paradigms of LLMs, the accurate measurement of their associated risks mandates a reconstruction of the LLMs' application scenarios (the conditioned contexts). For a precise evaluation of the discrimination risk posed by language models in practical settings, the test data we devise must thoroughly and accurately emulate the textual environment these models encounter. Foremost, the linguistic distribution in the test dataset should exhibit a close resemblance to that observed in the application scenarios. Additionally, the composition of the test data ought to be all-encompassing. A comprehensive audit of a model requires a detailed and diverse collection of test data for an accurate appraisal of discrimination risk, moving beyond a mere dependence on predetermined phrases or stereotypes indicative of bias. It is only in such rigorously designed testing conditions that the statistical information forecasted by the language model can authentically mirror the actual discrimination risk in application scenarios. Further more, discrimination risk is exclusively determined by the static system's prejudice and the change of specific context conditioned on (a.k.a. caprice), and the cost or risk of loss for these two elements varies depending on the application scenarios, like medical vs. legal and judicial, so it's necessary for the auditing framework to spilt them apart.



%Discrimination risk is exclusively determined by the static/general system's prejudice and the specific context its generation is conditioned on (a.k.a. caprice), and the cost or risk of loss for these two elements varies depending on the application scenarios, like medical vs. legal and judicial, so it's necessary for the auditing framework to spilt them apart.
\input{Figures/framework}

As illustrated in Figure \ref{fig:framework}, in this work, we present a statistical framework to measure social discrimination in LLMs, complemented with an automated \textit{context template} data-mining approach, as well as a mathematical perspective for risk decomposition related to LLMs’ \textit{prejudice} and \textit{caprice}. Practically speaking, we investigate the inductive bias of LLMs towards a demographical group $Y$ given another demographical group $X$ as the prior. This exploration involves statistically analyzing LLMs' predicted word probabilities conditioned on context templates augmented with $X$, whose distribution aligns with that of the applied contexts of LLMs. While our framework is adaptable to any assigned $X$ and $Y$, we exemplify it using \textit{occupations} as $X$ and \textit{binary gender}\footnote{We acknowledge diverse gender identities and employ a binary framework only for experimental consistency with prior research.} as $Y$ in our case study. More specifically, for the collection of context templates, we initially mine sentences from a large corpus, ensuring that these sentences contain words from both $X$ and $Y$ with coreference. Subsequently, we parse and document the structures of these sentences using syntactic trees, counting the obtained sentence skeletons to approximate the real distribution of context templates. We avoid crowd-sourced or LLM-generated context templates to prevent introducing prior biases from humans or other models. For risk decomposition, we attribute the risk arising from LLMs' \textit{prejudice} to the \textit{mean} of the calculated risk under a range of specific contexts, and the risk from LLMs' \textit{caprice} to the \textit{variance} of the same variable. Therefore, our framework serves as an exhaustive audit for evaluating social discrimination in LLMs, contributing to the communities’ collective efforts to develop transparent, fair, and reliable models.
% In order to mitigate the aforementioned limitations, this study introduces an innovative framework for assessing model discrimination risk. This framework employs a sampling method grounded in the linguistic context encountered by the model. It specifically selects texts pertaining to protected attributes such as gender and race through a process of coreference inference. Subsequently, these texts undergo a cleansing process using syntactic structures to develop a diverse array of templates. The model's biases towards protected attributes, such as gender and race, are extrapolated from the conditional probabilities it predicts across these varied templates. Such probability distributions serve as a mirror, reflecting the model's discriminatory proclivities. To quantify these observations, we have formulated specific risk measurement indicators that correspond to the predictions, thereby delineating the degree of bias present in the model's linguistic processing. This bias could emanate from two principal sources: stereotypes ingrained in the model during its training (systemic discrimination), or arbitrary unfair predictions stemming from the model's inherent unpredictability (random discrimination). By segmenting model discrimination into these two core categories, we enhance our capacity to precisely identify, comprehend, and dissect the model's unjust inclinations. Our framework, therefore, stands as a pivotal auditing instrument, facilitating the development of language models that are not only fairer and more transparent but also inherently reliable.

In addition, we apply our evaluation framework to 12 widely used language models, providing insights and issuing pre-warnings on the risk of employing potentially biased LLMs. Key points include: \textit{i)} all our examined models exhibits notable \textit{pro-male} bias, \textit{ii)} increasing the model size and incorporating human feedback in LLMs’ training doesn’t guarantee improved fairness, \textit{iii)} LLMs’ \textit{prejudice} contributes significantly to the application risk of larger models, and shows strong correlations with social and economic factors such as salary and education year, and \textit{iv)} the risk from LLMs’ \textit{caprice} follows a fat-tailed distribution, indicating a hard-to-predict \textit{wild risk} defying the law of large numbers, which requires strengthened surveillance and regulatory measures.
% An evaluation was conducted on the extent of discrimination in twelve extensively utilized pre-trained language models, substantiating the efficacy of our discrimination risk assessment framework. Our findings revealed that all the models under scrutiny exhibit a pronounced pro-male bias. Interestingly, it was observed that an increase in model parameters and the incorporation of human feedback learning do not invariably lead to enhanced fairness. Predominantly, systemic discrimination emerged as a significant factor contributing to the inequity of larger models, exhibiting a strong correlation with disparities in social and economic factors. Additionally, random discrimination was found to adhere to a fat-tailed distribution, representing a 'wild risk' that defies the law of large numbers and presents challenges in predictability, necessitating heightened vigilance and control measures.

==> introduction_legacy0217.tex <==
\section{Introduction}
\input{Figures/intuitive_understanding}

While large language models (LLMs) exhibit impressive world prior knowledge after being pre-trained on web-scaled data, they pose risks when applied to real-world tasks, as their generation may inadvertently perpetuate or amplify existing social discrimination present in the training data, potentially leading to unfair and even detrimental outcomes towards specific individuals or groups \citep{bolukbasi2016man,sheng2020nice,mei2023bias}. For instance, job matching systems powered by LLMs could unintentionally disadvantage ethnic minorities or individuals with disabilities \citep{hutchinson2020social}. Similarly, modern machine translation systems often transform gender-neutral terms into predominantly gendered forms, potentially intensifying existing gender biases  \citep{stanovsky-etal-2019-evaluating}. Consequently, the biased generation of LLMs might have adverse effects on critical decisions, such as those related to credit authorization, judicial decision-making, and healthcare, endangering individual rights and the fundamental principles of equality \citep{barocas2017problem,cowgill2018bias,deshpande2020mitigating,dressel2018accuracy,Reuters2018Amazon}.

Previous methods for assessing discrimination in LLMs \textit{merely} focused on their \textit{average discriminatory performance} over multiple test samples \citep{nadeem2020stereoset,nangia2020crows}, which has been shown to be inadequate due to the oversight of other crucial discrimination-leading factors. Multi-sample measurements are favored because any entity's preferences vary across \textit{contexts}\footnote{In the case of LLMs, \textit{contexts} refer to their textual operational settings, such as varied job requirements and candidate resumes for job matching, or diverse case keywords and legal databases for legal information retrieval.} (shown in Figure \ref{fig:intuitive_understanding}), necessitating substantial samples to capture persistently biased behavioral patterns. However, solely relying on the average behavior of the LLMs hampers accurate discrimination estimation in the following scenario:

\textit{Suppose the unbiased preference is $p^\star=(\textcolor{MALE_COLOR}{0.5}, \textcolor{FEMALE_COLOR}{0.5})$. We have two entities, $E_1$ and $E_2$, each displaying preferences in contexts $\{C_1, C_2\}$, with the corresponding preference errors and system biases computed as follows: }

\begin{center}
    $E_1: \{C_1: (\textcolor{MALE_COLOR}{0.6}, \textcolor{FEMALE_COLOR}{0.4}), C_2: (\textcolor{MALE_COLOR}{0.6}, \textcolor{FEMALE_COLOR}{0.4})\}, error=\textcolor{RISK_COLOR}{\textbf{20\%}}, system~bias=\textcolor{RISK_COLOR}{\textbf{0.1}}$;
\end{center}

\begin{center}
    $E_2: \{C_1: (\textcolor{MALE_COLOR}{0.7}, \textcolor{FEMALE_COLOR}{0.3}), C_2: (\textcolor{MALE_COLOR}{0.3}, \textcolor{FEMALE_COLOR}{0.7})\}, error=\textcolor{RISK_COLOR}{\textbf{40\%}}, system~bias=\textcolor{RISK_COLOR}{\textbf{0}}$.
\end{center}

\textit{where the system bias quantifies the difference between an entity's average contextualized preferences and the unbiased preference. }

While employing the average performance, i.e., system bias in this scenario, as a discrimination measure can be effective, it remains incomplete. This approach overlooks the variance of the entity's preferences, which reflects inconsistency and unpredictability in their predictions or decision-making. Such oversight can lead to measurement outcomes that defy intuitive understanding, as seen in this case of \textit{high error} but \textit{low system bias}. Consequently, a comprehensive quantitative measure of model discrimination should consider both \textit{average performance} and \textit{performance variance}, termed \textit{prejudice} and \textit{caprice} in our study, respectively.

Furthermore, prior studies often relied on manually generated content to construct datasets for discrimination detection, inevitably introducing human biases  \citep{nadeem2020stereoset,nangia2020crows}. Conversely, given that the discrimination measurement outcomes are intrinsically affected by the chosen context set, employing a set of bias-measuring context probes that approximates the LLMs' applied environments yields the most pragmatically meaningful results. As LLMs typically follow a language modeling paradigm throughout training and usage, they demonstrate \textit{preferences} by conditioned word probability prediction. Specifically, whether generating evaluation reports from job applicants' resumes \citep{gan2024application} or extracting legal information for judicial decisions \citep{wu2023precedent}, these models essentially develop responses implying their inductive biases by calculating and maximizing the probability of the next (or masked) tokens highly dependent on scenario-specific contexts. Therefore, evaluating the LLMs’ discrimination and application risk necessitates restoring their use cases because LLMs act as probability estimators for desired tokens conditioned on their deployment contexts. 

\input{Figures/framework}

As illustrated in Figure \ref{fig:framework}, we hereby introduce a Prejudice-Caprice Framework (PCF) to comprehensively measure social discrimination in LLMs, by considering not only the models’ \textit{consistent discriminatory performance} but also their \textit{performance variance across multiple contexts}, where the context collection is automated by a data-mining approach. Originally designed for measuring LLMs' discrimination, our proposed PCF allows statistical analysis and comparison of inductive biases, i.e. knowledge and prejudice, in any modal model, provided the framework's components are appropriately adapted for that use case (refer to Section \ref{sec:discussions} for more details). PCF exhibits the following properties: \textit{i)} an ideally unbiased model has an overall discrimination risk of 0, \textit{ii)} a randomly initialized model shows 0 prejudice risk but the highest caprice risk\footnote{In this paper, we use prejudice risk interchangeably with system risk, and caprice risk with efficiency risk.}, and \textit{iii)} a stereotyped model has the highest prejudice risk and 0 caprice risk.

Practically speaking, we investigate the inductive bias of LLMs towards a demographical group $Y$ given another demographical group $X$ as the evidence. This exploration involves statistically analyzing LLMs' predicted word probabilities conditioned on context templates augmented with $X$, whose distribution aligns with that of the applied contexts of LLMs. While our framework is adaptable to any assigned $X$ and $Y$, we exemplify it using \textit{occupations} as $X$ and \textit{binary gender}\footnote{We acknowledge diverse gender identities and employ a binary framework only for experimental consistency with prior research.} as $Y$ in our case study. More specifically, for risk decomposition, we attribute the risk arising from LLMs' \textit{prejudice} to the \textit{mean} of the calculated risk under a range of specific contexts, and the risk from LLMs' \textit{caprice} to the \textit{variance} of the same variable. For the collection of context templates, we initially mine sentences from a large corpus, ensuring that these sentences contain words from both $X$ and $Y$ with coreference. Subsequently, we parse and document the structures of these sentences using syntactic trees, counting the obtained sentence skeletons to approximate the real distribution of context templates. We avoid crowd-sourced or LLM-generated context templates to prevent introducing prior biases from humans or other models. Therefore, our framework serves as an exhaustive audit for evaluating social discrimination in LLMs, contributing to the communities’ collective efforts to develop transparent, fair, and reliable models.

We apply our evaluation framework to 12 widely used language models, providing insights and issuing pre-warnings on the risk of employing potentially biased LLMs. Key points include: \textit{i)} all our examined models exhibits notable \textit{pro-male} bias, \textit{ii)} LLMs’ \textit{prejudice} contributes significantly to the application risk of larger models, and shows strong correlations with social and economic factors such as salary and education year, and \textit{iii)} the risk from LLMs’ \textit{caprice} follows a fat-tailed distribution, indicating a hard-to-predict \textit{wild risk} defying the law of large numbers, which requires strengthened surveillance and regulatory measures.

% \textit{ii)} increasing the model size and incorporating human feedback in LLMs’ training doesn’t guarantee improved fairness, \textit{iii)} LLMs’ \textit{prejudice} contributes significantly to the application risk of larger models, and shows strong correlations with social and economic factors such as salary and education year, and \textit{iv)} the risk from LLMs’ \textit{caprice} follows a fat-tailed distribution, indicating a hard-to-predict \textit{wild risk} defying the law of large numbers, which requires strengthened surveillance and regulatory measures.

==> introduction_legacy0511.tex <==
\section{Introduction}
\input{Figures/intuitive_understanding}

While large language models (LLMs) exhibit impressive world prior knowledge after being pre-trained on web-scaled data, they pose risks when applied to real-world tasks, as their generation may inadvertently perpetuate or amplify existing social discrimination present in the training data, potentially leading to unfair and even detrimental outcomes towards specific individuals or groups \citep{bolukbasi2016man,sheng2020nice,mei2023bias}. For instance, job matching systems powered by LLMs could unintentionally disadvantage ethnic minorities or individuals with disabilities \citep{hutchinson2020social}. Similarly, modern machine translation systems often transform gender-neutral terms into predominantly gendered forms, potentially intensifying existing gender biases  \citep{stanovsky-etal-2019-evaluating}. Consequently, the biased generation of LLMs might have adverse effects on critical decisions, such as those related to credit authorization, judicial decision-making, and healthcare, endangering individual rights and the fundamental principles of equality \citep{barocas2017problem,cowgill2018bias,deshpande2020mitigating,dressel2018accuracy,Reuters2018Amazon}.

Previous methods for assessing discrimination in LLMs \textit{merely} focused on their \textit{average discriminatory performance} over multiple test samples \citep{nadeem2020stereoset,nangia2020crows}, which has been shown to be inadequate due to the oversight of other crucial discrimination-leading factors. Considering that any entity's preferences vary across \textit{contexts}\footnote{In the case of LLMs, \textit{contexts} refer to their textual operational settings, such as varied job requirements and candidate resumes for job matching, or diverse case keywords and legal databases for legal information retrieval.}, multi-sample measurements are favored as they enable assessment of both the \textit{mean} and \textit{variation} of the entity's biased behavioral pattern (shown in Figure \ref{fig:intuitive_understanding}). However, prior measurements that solely rely on the average behavior of the LLMs hampers accurate estimation in the following scenario:

\textit{Suppose the unbiased preference is $\mathbf{p}^\star=(\textcolor{MALE_COLOR}{0.5}, \textcolor{FEMALE_COLOR}{0.5})$. We have two entities, $E_1$ and $E_2$, each displaying preferences in contexts $\{C_1, C_2, C_3\}$, with the corresponding system biases and preference errors computed as follows: }

\begin{center}
    $E_1: \{C_1: (\textcolor{MALE_COLOR}{0.6}, \textcolor{FEMALE_COLOR}{0.4}), C_2: (\textcolor{MALE_COLOR}{0.6}, \textcolor{FEMALE_COLOR}{0.4}), C_3: (\textcolor{MALE_COLOR}{0.6}, \textcolor{FEMALE_COLOR}{0.4})\}, system~bias=\textcolor{RISK_COLOR}{\textbf{0.1}}, error=\textcolor{RISK_COLOR}{\textbf{20\%}}$;
\end{center}

\begin{center}
    $E_2: \{C_1: (\textcolor{MALE_COLOR}{0.5}, \textcolor{FEMALE_COLOR}{0.5}), C_2: (\textcolor{MALE_COLOR}{0.35}, \textcolor{FEMALE_COLOR}{0.65}), C_3: (\textcolor{MALE_COLOR}{0.65}, \textcolor{FEMALE_COLOR}{0.35})\}, system~bias=\textcolor{RISK_COLOR}{\textbf{0}}, error=\textcolor{RISK_COLOR}{\textbf{20\%}}$.
\end{center}

\textit{where the system bias quantifies the difference between an entity's average contextualized preferences and the unbiased preference. }

While employing the average performance, i.e., system bias in this scenario, as a discrimination measure can be effective, it remains incomplete. This approach overlooks the variation of the entity's preferences, which reflects inconsistency and unpredictability in their predictions or decision-making. Such oversight can lead to measurement outcomes that defy intuitive understanding, as seen in the case of $E_2$, which exhibits fluctuated biased preferences across contexts, yet its system bias remains at $\textcolor{RISK_COLOR}{\textbf{0}}$. Furthermore, \textit{error} alone cannot fully capture the biased behavior of the entity. For instance, comparing $E_1$ and $E_2$, while both have the same error to be $\textcolor{RISK_COLOR}{\textbf{20\%}}$, it does not account for the fact that the predictions of $E_2$ exhibit larger variations, and its preferences are more biased in certain contexts. Consequently, a comprehensive quantitative measure of model discrimination should \textit{i)} consider both \textit{average performance} and \textit{performance variation}, termed \textit{prejudice} and \textit{caprice} in our study, respectively; and \textit{ii)} facilitate their decomposition accordingly.

As LLMs typically follow a language modeling paradigm throughout training and usage, they demonstrate \textit{preferences} by conditioned word probability prediction. Specifically, whether generating evaluation reports from job applicants' resumes \citep{gan2024application} or extracting legal information for judicial decisions \citep{wu2023precedent}, these models essentially develop responses implying their inductive biases by calculating and maximizing the probability of the next (or masked) tokens highly dependent on scenario-specific contexts. Therefore, this conditional generation setup allows for the examination of how LLMs associate factors, such as occupation and gender, among others, provided they are given appropriate conditioned contexts.

\input{Figures/framework}

% implying the language model beneath is a unigram model
As illustrated in Figure \ref{fig:framework}, we hereby introduce a Prejudice-Caprice Framework (PCF) to comprehensively measure social discrimination in LLMs, by considering not only the models’ \textit{consistent discriminatory performance} but also their \textit{performance variation across multiple contexts}. Our framework stands out from previous methods because we correct a misconception that model bias resembles a biased coin toss or weighted dice roll. In these analogies, each context, just like any independent flip of a coin or roll of a dice, is assumed to be a homogeneous preference (i.e., word probabilities) elicitor, suggesting that preferences elicited are drawn from the same distribution and will not be affected by the given contexts. Instead, we propose \textit{heterogeneous contexts }to frame the assessment of discrimination. This entails acknowledging that models' predictions are not solely determined by their inbuilt inductive bias but also by the nuanced conditioned contextual cues, necessitating the collection of diverse contexts to quantify both preference persistence and fluctuations. Originally designed for measuring LLMs' discrimination, our proposed PCF allows statistical analysis and comparison of inductive biases, i.e. knowledge and prejudice, in any modal model, provided the framework's components are appropriately adapted for that use case (refer to Section \ref{sec:discussions} for more details). PCF exhibits the following properties: \textit{i)} an ideally unbiased model has an overall discrimination risk of 0, \textit{ii)} a stereotyped model has the highest prejudice risk and 0 caprice risk, and \textit{iii)} a randomly stereotyped model shows 0 prejudice risk but the highest caprice risk.

Practically speaking, we investigate the inductive bias of LLMs towards a demographical group $Y$ given another demographical group $X$ as the evidence. This exploration involves statistically analyzing LLMs' predicted word probabilities conditioned on context templates augmented with $X$, whose distribution aligns with that of the applied contexts of LLMs. It is noteworthy that $X$ and $Y$ could be instantiated for various measurement objectives, for example, $X$ as \textit{occupations} and $Y$ as \textit{gender} for assessing gender bias within each industry, or $X$ as \textit{education year} and $Y$ as \textit{income} for evaluating the impact of education on social stratification. 

More specifically, for risk decomposition, we attribute the risk arising from LLMs' \textit{prejudice} to the \textit{mean} of the calculated risk under a range of specific contexts, and the risk from LLMs' \textit{caprice} to the \textit{variation} of the same variable. For the automatic collection of context templates, we initially mine sentences from a large corpus, ensuring that these sentences contain words from both $X$ and $Y$ with coreference. Subsequently, we parse and document the structures of these sentences using syntactic trees, counting the obtained sentence skeletons to approximate the real distribution of context templates. We avoid crowd-sourced or LLM-generated context templates to prevent introducing prior biases from humans or other models. Therefore, our framework serves as an exhaustive audit for evaluating social discrimination in LLMs, contributing to the communities’ collective efforts to develop transparent, fair, and reliable models.

We apply our evaluation framework to 12 widely used language models, providing insights and issuing pre-warnings on the risk of employing potentially biased LLMs. Key points include: \textit{i)} all our examined models exhibit notable \textit{pro-male} bias, \textit{ii)} LLMs’ \textit{prejudice} contributes significantly to the application risk of larger models, and shows strong correlations with social and economic factors such as salary and education year, and \textit{iii)} the risk from LLMs’ \textit{caprice} follows a fat-tailed distribution, indicating a hard-to-predict \textit{wild risk} defying the law of large numbers, which requires strengthened surveillance and regulatory measures.

% \textit{ii)} increasing the model size and incorporating human feedback in LLMs’ training doesn’t guarantee improved fairness, \textit{iii)} LLMs’ \textit{prejudice} contributes significantly to the application risk of larger models, and shows strong correlations with social and economic factors such as salary and education year, and \textit{iv)} the risk from LLMs’ \textit{caprice} follows a fat-tailed distribution, indicating a hard-to-predict \textit{wild risk} defying the law of large numbers, which requires strengthened surveillance and regulatory measures.

==> modeling_copy.tex <==
\section{Mathematical Modeling }
\label{sec:mathematical_modeling_of_social_discrimination_and_risk_decomposition}
\input{Figures/risk_decomposition}
% TODO:
% * Explain Figure 2 with a simple binary gender setting (preference, J(p), r, $r_x$, and R) in the format of definition, meaning, and example.
% * Risk decomposition and its validity.
% * Emphasize math; binary gender illustration is only for easier readability.

We mathematically define the degree of a LLM's stereotype. We notice that the inconsistency of LLM's stereotype is induced by the variation of contexts. Further, LLMs predict the forthcoming tokens according to the tokens of the existed context. Therefore, our definition is based on the concept of LLM's token probability. When the LLM $M$ is applied to predict the type of the attribute $Y$ according to the index of a people group $X = x_i$ and other content of $C=c$, the model $M$ calculates the probabilities of all candidate tokens and selected the token having the highest predicted probability. Therefore, the token probabilistic nature caused LLM's inconsistency on stereotype. We denote the possible values of $Y$ as $y_1,y_2,\cdots,y_{|Y|}$, where $|Y|$ is the number of possible values for $Y$, and define $M$'s stereotype against $X = x_i$ about $Y = y_i$ in the context $C=c$ as follow:
\begin{equation}
    s_{x_i,y_i}^{M}(c) = \frac{p_{x_i,y_i}^M(c)}{p_{x_i,y_i}^*(c)}-1.
\end{equation}
We use $\mathbf{p}^*(c)=(p_1^*(c), p_2^*(c), \cdots, p_{|Y|}^*(c))$ to denote the probability when $M$'s unbiased. For instance, the unbiased probability of gender issue is $\mathbf{p}^*(c)=(0.5, 0.5)$. Once the context $c$ does not include information about the attribute $Y$, we set $p_1^*(c)=p_2^*(c)= \cdots= p_{|Y|}^*(c)= \frac{1}{|Y|}$. When $s_{x,y_1}>0$, it indicates that $Y=y_i$ is a stereotype of $X=x_i$; conversely, it represents an anti-stereotype. The absolute value of $s_{x,y_1}$ signifies the corresponding intensity. On the basis of $s_{x,y_1}$, we further define two indices to summarizing LLM's discrimination against group $X=x_i$ and summarizing LLM's overall discrimination levels for all people groups and all attributes. 
\begin{definition}
The Conditional Discrimination Risk $r_x$, measuring $M$'s discrimination risk against $X=x_i$ for all types of the attribute $Y$ is:
\begin{equation}
    r_x = \mathbb{E}_{c\sim C}(J(s_{x,y}^{M}(c))). \label{eq:r_x}
\end{equation}
We further define the concept of LLM's Overall Discrimination Risk to summarize $M$'s discrimination for all people groups about the attribute $Y$, which is:
\begin{equation}
    R = \mathbb{E}_{x\sim X}(r_x). \label{eq:R}
\end{equation}
\end{definition}
We emphasize that our definition about $s_{x,y}^{M}(c)$ is developed according to the definition about human being's stereotype degree in sociology literature. The sociologists have noticed that various persons have different stereotypes against the same group of people for any given attribute\citep{brigham1971ethnic, mccauley1980stereotyping}. Therefore, the sociology literature has defined the concept of degree of a person's stereotype by his/her belief about the correlation between a group of people and a specific attribute \citet{brigham1971ethnic, mccauley1980stereotyping}. In the Appendix, we further reviewed related studies. 



\iffalse
Two reasons drive us to mathematically define $s_{x_i,y_i}^{M}(C)$ on the basis of token probability of LLM. First, we note that the randomness of $s_{x_i,y_i}^{M}(C)$ is originated by the variation of $C$ for studied people-group $X=x_i$ and attribute type $Y=y_i$. Second, 


We first mathematically define the degree of a LLM's stereotype by combining the stereotype degree definition in sociology and the concept of LLM's token probability. The sociologists have noticed that various persons have different stereotypes against the same group of people for any given attribute\citep{brigham1971ethnic, mccauley1980stereotyping}. For instance, some people consider doctor as a feminine job while some other consider doctor as a masculine job. Evern among the people who all consider doctor as a feminine job, they can have different views about how strong the doctor job correlating with feminine characteristics. Therefore, the sociology literature has defined the concept of degree of a person's stereotype by his/her belief about the correlation between a group of people and a specific attribute \citet{brigham1971ethnic, mccauley1980stereotyping}, which is 
\begin{equation}
    s_{y,x} = \frac{P(Y=y|X=x)}{P(Y=y)}-1.
\end{equation}
Here, the random variable $X$ denotes the people group while the random variable $Y$ denotes the attribute type. $P(Y=y|X=x)$ denotes the person's believe about the probability that the group's attribute type $Y$ is $y$ when the group number is $X=x$. For instance, $P(Y = nurse)|X=female$ denotes the person's believe about the person's believe about the correlation between the job $nurse$ as an attribute with the female people. When $s_{y,x}$ is positive, the person's stereotype trend to label the group of people $X=x$ by attribute $Y=y$. When $s_{y,x}$ is positive, the person's stereotype considered that the group of people $X=x$ have other values of the attribute $Y$ rather than $y$. For instance, $s_{nurse,female}$ is negative, the people believe that the nurse is a masculine job. 

To adequately model LLM's attitude on social-justice topics. the above definition in sociology is adjusted according to LLM's inconsistent token-prediction nature. LLM's inconsistency caused that the same model $M$'s predictions about the correlation between people group and attribute type can vary by context $C$. Thus, the degree of $M$'s stereotype against the people-group $X$ about the protected attribute $Y$ is a random variable over context and denoted by $s_{X,Y}^{M}(C)$. 


%If there is no information about the protected attribute in the context $c$, then $p_1^*(c)=p_2^*(c)= \cdots= p_{|Y|}^*(c)= \frac{1}{|Y|}$. 

% Thus
% \begin{equation}
%     s_{x,y_i} = |Y|p_i-1 = |Y|p_i -\sum_{i=1}^{|Y|}p_i = < {d}_{y_i}, \mathbf{p} >,
%     \label{eq:S_y}
% \end{equation}
 %where $<\cdot,\cdot>$ is the inner product operator and 
% \begin{equation}
%      \mathbf{d}_{y_i} = \left( -1, -1, \ldots, |Y|-1, \ldots, -1 \right) \label{eq:d_y}
% \end{equation}
%  is the projection direction whose $i$th element is $|Y|-1$, while others are uniformly $-1$. Please refer to the Appendix for specific examples. We could use the stereotype vector to model the stereotype of $M$ of $Y$ can be represented by the vector 
%   \begin{equation}
%   \mathbf{s}_x^M(c)=(s_{x,y_1}(c), s_{x,y_2}(c), \cdots, s_{x,y_{|Y|}}(c)).
%   \end{equation}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\linewidth]{stereo_dist.png}
  \caption{Distribution of the stereotype.}
  \label{fig:dist}
\end{figure}

% 刻板印象受到cotext的随机性的影响表现为一个随机变量，其概率分布函数为：
% \begin{definition}\label{def:dist}
%    The degree of stereotype is influenced by the randomness of the context, manifesting as a random variable. Thus the probability distribution function of the degree of stereotype is defined as:
\begin{equation}
    F(a) = \mathbb{P}_{c\sim C}[s_{x,y}^{M}(c)<a].
\end{equation}
% \end{definition}

%以男性刻板印象为例，我们可以统计LLM的男性stereotype强度的概率密度函数，如图所示。特别地，y轴右侧概率密度函数的积分反映了LLM表现出男性刻板印象

%例如，以性别为例，。

%\textcolor{red}{we need a definition about stereotype distribution!}



%To adequately model LLM's attitude on social-justice topics in a particular context, we define the stereotype degree of model $M$ against the people-group $X$ about the protected attribute $Y$ in a particular context $C=c$. The stereotype degree is denoted by as $s_{x,y}^{M}(c)$, which represents degree about how strong that the model $M$ predicts the correlation between the group of people $X=x$ and the attribute $Y = y$. For instance the correlation between nurses and female gender.%, As shown in Figure \ref{fig:risk_decomposition}(left).
% 我们把$Y$可能的取值记作$y_1,y_2,\cdots,y_{|Y|}$,其中|Y|$ is the number of possible values for $Y$.
%Our definition about a model $M$'s stereotype degree follows the sociology's definition about human's stereotype degree. % The sociology literature has defined the degree of a person's stereotype by the person's belief about the correlation between $X$ and $Y$ \citet{brigham1971ethnic, mccauley1980stereotyping}. We thus defined $s_{x,y}^{M}(c)$ as the correlation between $X$ and $Y$ for $M$'s prediction in the context $c$. 

%Mathematically, we rigrously define $s_{x,y}^{M}(c)$ on the basis of token probability because that LLMs predict the forthcoming tokens according to the tokens of the existed context. When the LLM $M$ is applied to generate the context related with a group of people $X = x$, the model $M$ calculates the probabilities of all candidate tokens.% As shown in Figure \ref{fig:risk_decomposition}(middle). 
%We denote the possible values of $Y$ as $y_1,y_2,\cdots,y_{|Y|}$, where $|Y|$ is the number of possible values for $Y$. 
% 我们挑选出分别挑选出candidate tokens中与protected attribute $Y$相关的单次，并将它们依据Y的取值分为|Y|组。我们定义p_i^M(c)表示当M的预测与Y相关的前提下落在第i组的条件概率。
%From the candidate tokens, we select those related to the protected attribute $Y$, and divide them into $|Y|$ groups according to the specific values $y_1,y_2,\cdots,y_{|Y|}$ that they related to. For instance, when we consider the biological-gender stereotype, the token "he" will be divided to the group of masculine tokens. We define $p_i^M(c)$ to represent the conditional probability that they are related to $y_i$ under the condition that the predictions are related to the protected attribute $Y$. The model $M$'s stereotype degree about $X$ in the context $c$ on the $i$th value of $Y$ is
% We groups those candidate tokens according to their relation with the possible values of the social-justice related attribute $Y$. For instance, when we consider the biological-gender stereotype, $Y$ has two possible values. The candidate tokens are groups to $3$ types: the feminine tokens, the masculine tokens, and gender-neutral tokens. We use $\mathbf{p}=(p_1, p_2, \cdots, p_{|Y|},p_{|Y|+1})$ to denoted the probability of each group of candidate tokens, predicted by $M$. Here $|Y|$ is the number of possible values for $Y$. The model $M$'s stereotype degree about $X$ in the context $c$ on the $i$th value of $Y$ is

\fi








%We can calculate the stereotype $s_{y,x}$ of LLMs by projecting the token probabilities predicted by LLMs, as shown in Figure \ref{fig:risk_decomposition} (midle). LLMs model language by predicting unknown words based on the condition of known words. Hence, our framework relies on LLMs' word prediction probabilities, which we refer to as LLMs' prediction $\mathbf{p}=(p_1, p_2, \cdots, p_{|Y|})$, which is a probability distribution of words related to each protected attribute $Y$ correspondingly. Here $|Y|$ is the number of possible values for $Y$. The model's stereotype of the i-th item is
%\begin{equation}
%    s_{y,x} = \frac{p_M(Y|X;c)}{P(Y=y_i)}-1 = \frac{p_i}{P(Y=y_i)}-1.
%\end{equation}
%If there is no information about the protected attribute in the context, then $P(Y=y_1)=P(Y=y_2)=\cdots=P(Y=y_{|Y|})=\frac{1}{|Y|}$. Thus
%\begin{equation}
%    s_{y,x} = |Y|p_i-1 = |Y|p_i -\sum_{i=1}^{|Y|}p_i = < \mathbf{d}_Y, \mathbf{p} >,
%    \label{eq:S_y}
%\end{equation}
%where $<\cdot,\cdot>$ is the inner product operator and 
%\begin{equation}
%     \mathbf{d}_Y = \left( -1, -1, \ldots, |Y|-1, \ldots, -1 \right) \label{eq:d_y}
%\end{equation}
%  is the projection direction whose $y^{th}$ element is $|Y|-1$, while others are uniformly $-1$. Please refer to the Appendix for specific examples.
%Note that we define $s_{Y,X,M,C}$ on the basis of the definition about stereotype degree in the sociology literature. The socilogists have noticed that any two person can have different stereotype direction for people-group $X$ about attribute $Y$. For instance, 
%The  has noticed that two persons can have different degree 
%defined the degree of a person's stereotype for people-group $X$ about attribute $Y$ 
%noticed that people's stereotype has various degree 
%Due to the model inconsistency, $s_{Y,X,M,C}$ varies by $C$ for a given model $M$. 
%Stereotypes are characteristics that society instinctively attributes to groups of people to classify them according to age, weight, occupation, skin colour, gender, etc.



%Compared to human stereotypes, the LLMs' stereotypes possess randomness due to the inconsistency, as shown in Figure \ref{fig:risk_decomposition}. \citet{brigham1971ethnic, mccauley1980stereotyping} model personal stereotypes $s_{y,x}$ as probabilistic predictions of traits $Y=y$ based on information about group members $X=x$:
%\begin{equation}
%    s_{y,x} = \frac{P(Y=y|X=x)}{P(Y=y)}-1.
%\end{equation}
%When $s_{y,x}>0$, it indicates that $y$ is a stereotype of $x$; conversely, it represents an anti-stereotype \footnote{Building upon the method proposed by \citet{mccauley1980stereotyping}, where stereotypes are represented by $P(Y=y|X=x)/P(X=x)$, we have subtracted a constant of 1 to facilitate the distinction between stereotypes and anti-stereotypes through the sign.}. The absolute value of $s_{y,x}>0$ signifies the corresponding intensity. % Because context $c 会影响 the probabilistic predictions $p_M(Y|X;c)$ of LLMs, 所以LLM 产生的刻板印象$s_{y,x}$是一个随性来源于c的随机变量。
 %Because the context $c$ affects the probabilistic predictions $p_M(Y|X;c)$ of LLMs, the stereotype $s_{y,x}=\frac{p_M(Y|X;c)}{P(Y=y)}-1$ generated by LLMs is a random variable that arises from the randomness inherent in $c$, as shown in Figure \ref{fig:risk_decomposition} (left).

% 我们可以通过对LLMs 预测的token概率进行投影计算LLM的刻板印象$s_{y,x}$。现在的大语言模型通过预测给定句子时token的概率进行语言建模。在这里我们只关心与刻板印象有关联的词语的预测，不妨假设$u_1,$。
%We can calculate the stereotype $s_{y,x}$ of LLMs by projecting the token probabilities predicted by LLMs, as shown in Figure \ref{fig:risk_decomposition} (midle). LLMs model language by predicting unknown words based on the condition of known words. Hence, our framework relies on LLMs' word prediction probabilities, which we refer to as LLMs' prediction $\mathbf{p}=(p_1, p_2, \cdots, p_{|Y|})$, which is a probability distribution of words related to each protected attribute $Y$ correspondingly. Here $|Y|$ is the number of possible values for $Y$. The model's stereotype of the i-th item is
%\begin{equation}
%    s_{y,x} = \frac{p_M(Y|X;c)}{P(Y=y_i)}-1 = \frac{p_i}{P(Y=y_i)}-1.
%\end{equation}
%If there is no information about the protected attribute in the context, then $P(Y=y_1)=P(Y=y_2)=\cdots=P(Y=y_{|Y|})=\frac{1}{|Y|}$. Thus
%\begin{equation}
%    s_{y,x} = |Y|p_i-1 = |Y|p_i -\sum_{i=1}^{|Y|}p_i = < \mathbf{d}_Y, \mathbf{p} >,
%    \label{eq:S_y}
%\end{equation}
%where $<\cdot,\cdot>$ is the inner product operator and 
%\begin{equation}
%     \mathbf{d}_Y = \left( -1, -1, \ldots, |Y|-1, \ldots, -1 \right) \label{eq:d_y}
%\end{equation}
%  is the projection direction whose $y^{th}$ element is $|Y|-1$, while others are uniformly $-1$. Please refer to the Appendix for specific examples.

%\subsection{Measure the risk of LLM-induced discrimination}
% Gotoh, J.-y., and Uryasev, S. Approximation of Euclidean norm by Lp-representable norms and applications. University of Florida, Research Re- port 2013-3 (May 2013). http://www.ise.ufl.edu/uryasev/files/2013/06/ ApproxL2withLinearNorms.pdf.
% Pavlikov, K., and Uryasev, S. CVaR Norm and Applications in Optimization. University of Florida, Research Report 2013-1 (September 2013). http://www.ise. ufl.edu/uryasev/files/2013/08/cvar_norm_working_paper.pdf.

% 我们需要定义一个风险指标作为模型的歧视度量，而不能直接Stereotype dgree，which is a 依赖于contex随机性的随机变量。我们采用conditional value at risk (CVaR) norm对进行模型的歧视风险进行度量，如下面的定义所示
%To accurately quantify the level of bias in a model, we must establish a risk indicator rather than directly using the stereotype vector $\mathbf{s}_x^M(C)$, which is a random variable dependent on the context $C$'s randomness. There are three primary reasons: 1) 我们需要关注stereotype的影响，排除anti-stereotype的影响，which 已经反应在对其他$y$的刻板印象当中 2) 我们需要综合考虑模型对$y_1,y_2,\cdots,y_n$不同的刻板印象情况; 1) 我们需要综合考虑不同context下模型的综合表现。

The inconsistent nature of LLM's stereotype degree asks for a probabilistic way of measuring LLM's discrimination and the associated risk threatening the respective social justice. According to Def XXX, we measure LLM $M$'s discrimination against the group of people $X=x$ about the attribute type $Y=y_i$ by the conditional expectation of $s_{x,y_i}^{M}(c)$ that has positive value. Note that the LLM $M$ has different discrimination levels against the people group $x$ for all attribute types $y_1,y_2,\cdots,y_n$. For instance, the LLM $M$ has various discrimination levels against the females for all jobs such as nurse, doctor, etc. LLM's discrimination against a group of people for any attribute type $y_i$ must cause a social-injustice consequence. Therefore, to measure LLM's overall risk hurting a group of people in a specific social topic, we have to develop a metric that can summarize its discrimination against the same group of people for all types of the attribute related with the social topic. For instance, to capture LLM's overall threatening to female in job market, the measure metric has to summarize the model's discrimination against female for all careers. Following the risk-assessment literature about measuring overall risk that the same hazard causing multi-dimensional damages, we develop the concept of the maximal risk induced by $M$'s discrimination against people group $x$ for the attribute $Y$. 

%\begin{definition}
%The Discrimination Risk Criterion $J$, measuring the maximal stereotype degree of $M$:
%\begin{equation}
%    J(s_{x,y}^{M}(c))= \max_{y \in Y}\{s_{x,y}^{M}(c)^+\} \label{eq:J}
%\end{equation}
%where $s_{x,y}^{M}(c)^+ = \max{s_{x,y}^{M}(c),0}$ refers to the positive part of $s_{x,y}^{M}(c)$. The purpose of utilizing the positive part is to eliminate the interference of anti-stereotypes.
%\end{definition}

% Certainly, there are numerous definitions for $J(\mathbf{p})$, and its convexity governs the later decomposition outcomes. For example, the one presented in Equation \ref{eq:J} computes the \textit{infinity-norm} of the matrix $[s_{x,y}^{M}(c)^+]_{|Y|\times 1}$. Unlike other norms like the \textit{0-norm}, which counts non-zero elements, or the \textit{1-norm}, which sums the absolute values of matrix elements, this definition, due to its stronger convexity, emphasizes the portion of risk caused by the model's caprice. The proof can be found in Appendix \ref{app:J}.

\begin{definition}
The Discrimination Risk $r_x$ on group $X=x$ measuring by $L^n$ norm is defined as 
\begin{equation}
    r_x = \mathbb{E}_{c\sim C}[||\mathbf{s}_x^M(c)^{+}||_n]  \label{eq:J}
\end{equation}
The value of $r_x$ reflects the expected magnitude of $M$'s stereotypes against the group $x$ about the attribute type $y_i$.
where $\mathbf{s}_x^M(c)^+$ refers to the positive part\footnote{The positive part of a function $ f $, denoted as $ f^+ $, represents the part of $ f $ that is positive, i.e. $ f^+(x) = \max\{f(x), 0\} $.} of $\mathbf{s}_x^M(c)$ and $||\cdot||_n$ is the $L^n$ norm.
\end{definition}
Note that the maximal risk is one type of the $L^n$-norm metrics developed by the risk-assessment literature. According to the degree of public risk tolerance, the risk level can be measured by the associated $L^n$-norm metrics. The lower the acceptance, the larger the value of $n$. Here, we select the maximal risk that is $L^\infty$-norm metric because that the society shall have the minimal risk tolerance for LLM's discrimination considering its future impacts. 



To accurately quantify LLMs' discrimination, we establish a risk measurement rather than directly using the stereotype vector $\mathbf{s}_x^M(C)$. There are three primary reasons: 1) We need to focus on the impact of stereotypes while excluding anti-stereotypes, which is already reflected in the stereotypes towards other $y$ values;
2) We need to consider stereotypes for all possible attribute $y_1,y_2,\cdots,y_n$; 3) We need to take into account the model's overall performance across various contexts. Therefore, we present the following definition of Discrimination Risk.
% We employ the Conditional Value at Risk (CVaR) norm to measure the model's discrimination risk, as outlined in the definition below.




% rx反映了LLM对群体x产生刻板印象的整体风险大小。其中positive part让度量关注在stereotype上，Lp范数综合考虑了degree of 不同类型刻板印象，期望衡量了在不同context下模型的平均水平。
%LP范式的选择反映了。例如，l1，linfty。
The discrimination risk $r_x$ reflects the risk magnitude of the LLM's stereotypes about group $x$. %, As shown in Figure \ref{fig:risk_decomposition}(right). 
The positive part focuses the measure on stereotypes, the $L^n$ norm takes degree of various types of stereotypes into account the , and the expectation measures the model's average level across different contexts. The choice of $L^n$ norm indicates the degree of risk aversion. Specifically, as the value of $n$ increases, it signifies a higher level of individual aversion to uncertainty and risk, that is, a stronger degree of risk aversion. Conversely, a smaller value of $n$ suggests that the individual is more willing to accept risk. The detail explanation can be found in Appendix \ref{app:J}. Due to the maximal aversion to stereotypes, we choose $L^\infty$ norm in Equation \ref{eq:J} and all results in this paper are calculated by $L^\infty$ norm. 

Specifically, we can calculate the Overall Discrimination Risk posed by the LLM to all groups $x\sim X$, denoted as $R$, by
\begin{equation}
    R = \mathbb{E}_{x\sim X}(r_x). \label{eq:R}
\end{equation}

% Certainly, there are numerous choice for $L^n$ norm, which  its convexity governs the later decomposition outcomes. For example, the one presented in Equation \ref{eq:J} computes the \textit{infinity-norm} of the matrix $[S_y^+]_{|Y|\times 1}$. Unlike other norms like the \textit{0-norm}, which counts non-zero elements, or the \textit{1-norm}, which sums the absolute values of matrix elements, this definition, due to its stronger convexity, emphasizes the portion of risk caused by the model's caprice. The detail explanation can be found in Appendix \ref{app:J}.

% As $J$ is computed using the positive part of the stereotype $S_y$, its values are restricted to positive real numbers $ \mathbb{R}_+$. In line with the previous example, $J(\mathbf{p})$ is now $0.6$.
\subsection{Decompose LLM's discrmination to clarify AI Prejudice from AI Volatility}

% Just as human behavior adapts to varying environmental stimuli, the language understanding and generation of LLMs also fluctuate with subtle contextual shifts \citep{li2023nuances,li2024mutation}. 
%In extreme cases, model inconsistencies can lead to severe societal consequences \citep{dahan2023lawyers,nastasi2023vignette,chougule2023comprehensive}.
% 模型的歧视风险可能由两部分造成：1）2）。
% 这两类不同原因造成的风险，其对应的形成机制和治理方法都有差异。

Probabilistically modeling LLM's inconsistent stereotype degree manifests the two driven forces causing LLM's discrimination. One driven force is the estimation bias of LLM's prediction about the correlation between the group of people of a type of a specific attribute. The other driven force is the estimation variation. In statistics, the estimation bias implies that the LLM systematically connects the people group with the attribute type. In contrast, the estimation variation of the stereotype degree is an index of the LLM's estimation efficiency. The bias reflects the LLM's belief obtained from training by data while the variation reflects how vague the LLM's belief is. In statistics, the bias must be adjustable by modify the LLM architecture and training process. In contrast, the variation is not necessarily avoidable. 

Thus, decomposing LLM's discrimination risk according to the contributions of the bias and variation can verify how much the risk can be avoided. Meanwhile, the bias-induced discrimination can be considered as the LLM's prejudice while the variation induced part is LLM's vagueness. 
%We decompose the LLM's discrimination risk defined in Def XX into two part: the biased-induced part refereed as the prejudice risk and the variation-induced part refereed as volatility risk. 
%The aggregated contextualized discrimination risk of LLMs is divided into two components: prejudice, which arises from LLMs' systematic bias, and  volatility, which is due to their inconsistent output. The risks caused by these two different reasons have distinct formation mechanisms and governance methods.
%Therefore, we should focus on both the average performance and the performance variation across contexts, i.e., their generation's consistency and robustness. Drawing from this, we propose decomposing discrimination risk into parts attributed to persistent model prejudice and those resulting from their volatility.
\begin{definition}
The Prejudice Risk $r_x^p$ is the risk caused by the systemic estimation bias of LLM's estimation about the correlation between people-group $X$ and attribute $Y$.
\begin{equation}
    r_x^p =J(\mathbb{E}_{c~C}(s_{x,y}^{M}(c))).
    \label{eq:r_x^p}
\end{equation}
The Volatility Risk $r_x^v$ assesses $M$'s vagueness about its discrimination risk and is defined as :%caused by model inconsistencies and randomness besides the average stereotype, reflecting inadequate system robustness on group $X=x$:
\begin{equation}
    r_x^v = r_x - r_x^p \label{eq:r_x^c}
\end{equation}
\end{definition}
For all groups $x\sim X$, we could
 calculate the Overall Prejudice Risk $R^p$ and the Overall Volatility Risk $R^v$ by
\begin{equation}
    R^p = \mathbb{E}_{x\sim X}(r_x^p),
    R^v = \mathbb{E}_{x\sim X}(r_x^c). \label{eq:R^p}
\end{equation}

% For $r_x^p$, we initially compute the model's consistent preference for $x$, then evaluate the discrimination risk caused by this contextually constant bias with criterion $J$. Subsequently, the difference between $r_x$ and $r_x^p$, denoted as $r_x^c$, is attributed to the model's capricious behavior.

\iffalse

\begin{definition}
The Overall Discrimination Risk $R$, Overall Prejudice Risk $R^p$, and Overall Caprice Risk $R^c$, quantifying the model's global discriminatory behavior:
\begin{equation}
    R^p = \mathbb{E}_{x\sim X}(r_x^p) \label{eq:R^p}
\end{equation}
\begin{equation}
    R^c = \mathbb{E}_{x\sim X}(r_x^c) \label{eq:R^c}
\end{equation}
where each term represents the aggregation of the corresponding conditional risks across $X$.
\end{definition}




Today's LLMs are engineered to model vast textual data, typically with the language modeling objective. One common approach is the autoregressive language modeling, where we optimize parameters $\Theta$ of LLM $M_\Theta$ on a text corpus $U=\{u_1, \ldots, u_n\}$ by minimizing the loss function $L(U)=\sum_{i=1}^n \log P(u_i|u_1, \ldots, u_{i-1};\Theta)$. Expanding on the statistical insight that ``a word's meaning is shaped by its common co-occurrence with other words,'' optimizing language modeling objectives involves refining a series of conditional probabilities. This process continuously conditions on known words to predict unknown ones, shaping the entire training and application of the LLMs. LLMs' knowledge and prejudices, essentially their \textit{inductive biases}, are thus empirically revealed in their word predictions. Hence, our framework relies on LLMs' word prediction probabilities, which we refer to as LLMs' \textit{preferences} $\mathbf{p}$ (essentially a probability distribution of each protected attribute), forming the basis for our definitions of \textit{stereotypes} and \textit{risks} associated with social discrimination.

In a case study, we aim to investigate whether the model exhibits bias regarding gender $Y$ when conditioned on occupation $X$, such as persistently associating doctor/nurse with the \textcolor{MALE_COLOR}{male}/\textcolor{FEMALE_COLOR}{female}. Given context templates $T$ with distributions, occupation terms $X$ with distributions, and a set of gender-specific terms $Y$, we derive the LLM's gender-relevant preferences calibrated on $Y$ using $\mathbf{p}_{t, x} = M_{\Theta}(Y|t, x)$, where $t \sim T$ and $x \sim X$. As an illustration, suppose an LLM assigns an 80\% probability for $x$ being \textcolor{MALE_COLOR}{male} and a 20\% probability for it being \textcolor{FEMALE_COLOR}{female}. Thus, $\mathbf{p}=(\textcolor{MALE_COLOR}{0.8},\textcolor{FEMALE_COLOR}{0.2})$.

As depicted in Figure \ref{fig:risk_decomposition}, we measure social discrimination in LLMs starting from $\mathbf{p}$, transforming it into stereotypes $s$ or discrimination risks $r$ with different interpretations of this variable. We first introduce a supplementary concept of the \textit{stereotype projection direction} $\mathbf{d}_y$, with which we project preference $\mathbf{p}$ onto stereotype $s$ for category $y$ in $Y$. This direction is a multi-dimensional vector of length $|Y|$ and is determined based on the unbiased preference $\mathbf{p^\star}$. If $\mathbf{p^\star}$ is uniformly distributed across categories in $Y$, i.e. assigning equal chance to different $y$, $\mathbf{d}_y$ can be expressed as:

\begin{equation}
     \mathbf{d}_y = \left( -\frac{1}{|Y|-1}, -\frac{1}{|Y|-1}, \ldots, 1, \ldots, -\frac{1}{|Y|-1} \right) \label{eq:d_y}
\end{equation}


where the $y^{th}$ element is 1, while others are uniformly $-\frac{1}{|Y|-1}$.

With projection direction $\mathbf{d}_y$, the stereotype is defined as the inner product of $\mathbf{d}_y$ and $\mathbf{p}$:

\begin{equation}
    S_y = < \mathbf{d}_y, \mathbf{p} > \label{eq:S_y}
\end{equation}

We provide the characterization of $S_y$ and $\mathbf{d}_y$ in Appendix \ref{app:S_y}. For the gender setting of $Y$, if we set $\mathbf{d}_{masculine}=(1, -1)$ and $\mathbf{d}_{feminine}=(-1, 1)$, that would result in $S_{masculine}=0.6$ and $S_{feminine}=-0.6$ when $\mathbf{p}=(\textcolor{MALE_COLOR}{0.8},\textcolor{FEMALE_COLOR}{0.2})$. A persistent pattern of the LLM's preferences is observed when the values of all $S_y$ across $T$ with fixed $X=x$ tilts to one side, such as the \textit{pro-male stereotype} illustrated in the left side of Figure \ref{fig:risk_decomposition}.

\begin{definition}
The Discrimination Risk Criterion $J$, measuring the disparity between the model's preference $\mathbf{p}$, and the completely unbiased preference $\mathbf{p}^\star$:
\begin{equation}
    J(\mathbf{p})= \max_{y \in Y}\{S_y^+\} \label{eq:J}
\end{equation}
where $S_y^+$ refers to the positive part\footnote{The positive part of a function $ f $, denoted as $ f^+ $, represents the part of $ f $ that is positive, i.e. $ f^+(x) = \max\{f(x), 0\} $.} of $S_y$.
\end{definition}

Certainly, there are numerous definitions for $J(\mathbf{p})$, and its convexity governs the later decomposition outcomes. For example, the one presented in Equation \ref{eq:J} computes the \textit{infinity-norm} of the matrix $[S_y^+]_{|Y|\times 1}$. Unlike other norms like the \textit{0-norm}, which counts non-zero elements, or the \textit{1-norm}, which sums the absolute values of matrix elements, this definition, due to its stronger convexity, emphasizes the portion of risk caused by the model's caprice. The proof can be found in Appendix \ref{app:J}.

As $J$ is computed using the positive part of the stereotype $S_y$, its values are restricted to positive real numbers $ \mathbb{R}_+$. In line with the previous example, $J(\mathbf{p})$ is now $0.6$.
% The stereotype projection direction, projecting preference $p$ to discrimination risk $r$ and denoted as $y \in Y$, is characterized by a multi-dimensional vector of length $|Y|$. This can be mathematically expressed as follows:
% \begin{equation}
%     d_{y} = \left( -\frac{1}{|Y|-1}, -\frac{1}{|Y|-1}, \ldots, 1, \ldots, -\frac{1}{|Y|-1} \right)\label{eq:d_y}
% \end{equation}
% wherein the $y^{th}$ element is designated as 1, whilst the remaining elements are uniformly assigned the value $-\frac{1}{|Y|-1}$.


% \begin{equation}
%     J_y(p)=max\{<p, d_{y}>, 0\} \label{eq:J_y}
% \end{equation}
% where $<p, d_{y}>$ is the inner product of probability distribution prediction $p$ and discriminatory direction $d_y$.



\begin{definition}
The Conditional Discrimination Risk $r_x$, measuring the discrimination risk of  applying the model under the condition of fixed $X=x$:
\begin{equation}
    r_x = \mathbb{E}_{t\sim T}(J(\mathbf{p}_{t, X=x})) \label{eq:r_x}
\end{equation}
\end{definition}

$r_x$ computes the expected contextualized discrimination risk across diverse applied contexts under the fixed condition that $X = x$. For example, when occupation $X$ is set to $x$, $r_x$ quantifies the model's gender discrimination risk across contexts for occupation $x$. Comparing $r_x$ values helps comparatively assess gender discrimination risk among different occupations, thereby enabling inference about industries more susceptible to gender discrimination incidents.

Just as human behavior adapts to varying environmental stimuli, the language understanding and generation of LLMs also fluctuate with subtle contextual shifts \citep{li2023nuances,li2024mutation}. In extreme cases, model inconsistencies can lead to severe societal consequences \citep{dahan2023lawyers,nastasi2023vignette,chougule2023comprehensive}. Therefore, given the increasing integration of large foundation models into real-world applications to enhance social productivity, assessing their applicability should not only focus on the \textit{average performance} but also consider their \textit{performance variation} across contexts, i.e., their generation's consistency, predictability, robustness, and generalizability. Drawing from this, we propose decomposing discrimination risk into parts attributed to persistent model prejudice and those resulting from their behavioral inconsistencies.

\begin{definition}
The Conditional Prejudice Risk $r_x^p$ quantifying the model's discrimination risk resulting from its parametric prejudice when fixing $X=x$:
\begin{equation}
    r_x^p = J(\mathbb{E}_{t\sim T}(\mathbf{p}_{t, X=x})) \label{eq:r_x^p}
\end{equation}
and the Conditional Caprice Risk $r_x^c$, assessing the model's discrimination risk stemming from inconsistencies and randomness in its generation, reflecting inadequate system robustness when fixing $X=x$:
\begin{equation}
    r_x^c = r_x - r_x^p \label{eq:r_x^c}
\end{equation}

\end{definition}

For $r_x^p$, we initially compute the model's consistent preference for $x$, then evaluate the discrimination risk caused by this contextually constant bias with criterion $J$. Subsequently, the difference between $r_x$ and $r_x^p$, denoted as $r_x^c$, is attributed to the model's capricious behavior.

\begin{definition}
The Overall Discrimination Risk $R$, Overall Prejudice Risk $R^p$, and Overall Caprice Risk $R^c$, quantifying the model's global discriminatory behavior:
\begin{equation}
    R = \mathbb{E}_{x\sim X}(r_x) \label{eq:R}
\end{equation}
\begin{equation}
    R^p = \mathbb{E}_{x\sim X}(r_x^p) \label{eq:R^p}
\end{equation}
\begin{equation}
    R^c = \mathbb{E}_{x\sim X}(r_x^c) \label{eq:R^c}
\end{equation}
where each term represents the aggregation of the corresponding conditional risks across $X$.
\end{definition}

\fi

==> modeling_lyr.tex <==
\section{Mathematical Modeling }
\label{sec:mathematical_modeling_of_social_discrimination_and_risk_decomposition}
\input{Figures/risk_decomposition}
% TODO:
% * Explain Figure 2 with a simple binary gender setting (preference, J(p), r, $r_x$, and R) in the format of definition, meaning, and example.
% * Risk decomposition and its validity.
% * Emphasize math; binary gender illustration is only for easier readability.

\subsection{Stereotype distribution of LLMs and discrimination assessment}

% As shown in the middle plot of Figure \ref{fig:risk_decomposition}, 
%We first mathematically define the degree of a LLM's stereotype by combining the stereotype degree definition in sociology and the theory of token probability. The sociologists have noticed that various persons have different stereotypes against the same group of people for any given attribute\citep{brigham1971ethnic, mccauley1980stereotyping}. For instance, some people consider doctor as a feminine job while some other consider doctor as a masculine job. Evern among the people who all consider doctor as a feminine job, they can have different views about how strong the doctor job correlating with feminine characteristics. Therefore, the sociology literature has defined the concept of degree of a person's stereotype by his/her belief about the correlation between a group of people and a specific attribute \citet{brigham1971ethnic, mccauley1980stereotyping}, which is 
%\begin{equation}
%  s_{y,x} = \frac{P(Y=y|X=x)}{P(Y=y)}-1.
%\end{equation}



%Sociologists have defined personal stereotypes as probabilistic predictions that distinguish one group based on protected attribute \citep{brigham1971ethnic, mccauley1980stereotyping}. To adequately model LLM's stereotype,  LLM's inconsistency caused its predictions vary by context $C$. 
%The stereotype of LLMs exhibits randomness across different contexts, caused by their inherent inconsistency. It is imperative to address the randomness.
When the LLM $M$ is applied to predict the protected attribute $Y$ according to the index of people group $X = x$ under the content $C=c$, the model $M$ calculates the probabilities of all candidate tokens. We define $p_{x,y}^M(c)$ to represent the conditional probability that $M$ predict the $Y=y$ given $X=x$. Drawing from sociological definitions of stereotypes \citep{brigham1971ethnic, mccauley1980stereotyping}, we define the degree of $M$'s stereotype for $X=x$  with respect to the protected attribute $Y=y$ as:
\begin{equation}
    s_{x,y}^{M}(c) = \frac{p_{x,y}^M(c)}{p_{x,y}^*(c)}-1,
\end{equation}
where $p_{x,y}^*(c)$ denotes the unbiased probability. For instance, the unbiased probability of binary gender is $p_{x,male}^*(c)=p_{x,female}^*(c)=0.5$.  When $s_{y,x}$ is positive, the person's stereotype trend to label the group of people $X=x$ by attribute $Y=y$. When $s_{y,x}$ is positive, the person's stereotype considered that the group of people $X=x$ have other values of the attribute $Y$ rather than $y$. For instance, if $s_{nurse,female}$ is negative, the people believe that the nurse is a masculine job. %注意到受到context随机性的影响，s_{x,y}^{M}(c)是一个随机变量，图1给出了其概率密度函数的事例。

\begin{definition}
The Discrimination Risk Criterion $J$, measuring the maximal stereotype degree of $M$:
\begin{equation}
    J(s_{x,y}^{M}(c))= \max_{y \in Y}\{s_{x,y}^{M}(c)^+\} \label{eq:J}
\end{equation}
where $s_{x,y}^{M}(c)^+ = \max{s_{x,y}^{M}(c),0}$ refers to the positive part of $s_{x,y}^{M}(c)$. The purpose of utilizing the positive part is to eliminate the interference of anti-stereotypes.
\end{definition}

Certainly, there are numerous definitions for $J(\mathbf{p})$, and its convexity governs the later decomposition outcomes. For example, the one presented in Equation \ref{eq:J} computes the \textit{infinity-norm} of the matrix $[s_{x,y}^{M}(c)^+]_{|Y|\times 1}$. The detail explanation can be found in Appendix \ref{app:J}.% Unlike other norms like the \textit{0-norm}, which counts non-zero elements, or the \textit{1-norm}, which sums the absolute values of matrix elements, this definition, due to its stronger convexity, emphasizes the portion of risk caused by the model's caprice. The proof can be found in Appendix \ref{app:J}.


% We denote the possible values of $Y$ as $y_1,y_2,\cdots,y_{|Y|}$, where $|Y|$ is the number of possible values for $Y$, and define $M$'s stereotype against $X = x$ about $Y = y_i$ in the context $C=c$ as follow:

%To adequately model LLM's stereotype,  LLM's inconsistency caused that the same model $M$'s predictions vary by context $C$. Thus, the degree of $M$'s stereotype against the people-group $X$ about the protected attribute $Y$ is a random variable over context and denoted by $s_{X,Y}^{M}(C)$. 

Two reasons drive us to mathematically define $s_{x,y}^{M}(C)$ on the basis of token probability of LLM. First, we note that the randomness of $s_{x,y}^{M}(C)$ is originated by the variation of $C$ for studied people-group $X=x$ and attribute type $Y=y$. Second, LLMs predict the forthcoming tokens according to the tokens of the existed context. 

% Here, the random variable $X$ denotes the people group while the random variable $Y$ denotes the attribute type. 

 

% When $s_{x,y_1}>0$, it indicates that $Y=y_i$ is a stereotype of $X=x$; conversely, it represents an anti-stereotype. The absolute value of $s_{x,y_1}$ signifies the corresponding intensity.  
%If there is no information about the protected attribute in the context $c$, then $p_1^*(c)=p_2^*(c)= \cdots= p_{|Y|}^*(c)= \frac{1}{|Y|}$. 

% Thus
% \begin{equation}
%     s_{x,y_i} = |Y|p_i-1 = |Y|p_i -\sum_{i=1}^{|Y|}p_i = < {d}_{y_i}, \mathbf{p} >,
%     \label{eq:S_y}
% \end{equation}
 %where $<\cdot,\cdot>$ is the inner product operator and 
% \begin{equation}
%      \mathbf{d}_{y_i} = \left( -1, -1, \ldots, |Y|-1, \ldots, -1 \right) \label{eq:d_y}
% \end{equation}
%  is the projection direction whose $i$th element is $|Y|-1$, while others are uniformly $-1$. Please refer to the Appendix for specific examples. We could use the stereotype vector to model the stereotype of $M$ of $Y$ can be represented by the vector 
%   \begin{equation}
%   \mathbf{s}_x^M(c)=(s_{x,y_1}(c), s_{x,y_2}(c), \cdots, s_{x,y_{|Y|}}(c)).
%   \end{equation}

% 刻板印象受到cotext的随机性的影响表现为一个随机变量，其概率分布函数为：
% \begin{definition}\label{def:dist}
%    The degree of stereotype is influenced by the randomness of the context, manifesting as a random variable. Thus the probability distribution function of the degree of stereotype is defined as:
% \end{definition}

%以男性刻板印象为例，我们可以统计LLM的男性stereotype强度的概率密度函数，如图所示。特别地，y轴右侧概率密度函数的积分反映了LLM表现出男性刻板印象

%例如，以性别为例，。

%\textcolor{red}{we need a definition about stereotype distribution!}



%To adequately model LLM's attitude on social-justice topics in a particular context, we define the stereotype degree of model $M$ against the people-group $X$ about the protected attribute $Y$ in a particular context $C=c$. The stereotype degree is denoted by as $s_{x,y}^{M}(c)$, which represents degree about how strong that the model $M$ predicts the correlation between the group of people $X=x$ and the attribute $Y = y$. For instance the correlation between nurses and female gender.%, As shown in Figure \ref{fig:risk_decomposition}(left).
% 我们把$Y$可能的取值记作$y_1,y_2,\cdots,y_{|Y|}$,其中|Y|$ is the number of possible values for $Y$.
%Our definition about a model $M$'s stereotype degree follows the sociology's definition about human's stereotype degree. % The sociology literature has defined the degree of a person's stereotype by the person's belief about the correlation between $X$ and $Y$ \citet{brigham1971ethnic, mccauley1980stereotyping}. We thus defined $s_{x,y}^{M}(c)$ as the correlation between $X$ and $Y$ for $M$'s prediction in the context $c$. 

%Mathematically, we rigrously define $s_{x,y}^{M}(c)$ on the basis of token probability because that LLMs predict the forthcoming tokens according to the tokens of the existed context. When the LLM $M$ is applied to generate the context related with a group of people $X = x$, the model $M$ calculates the probabilities of all candidate tokens.% As shown in Figure \ref{fig:risk_decomposition}(middle). 
%We denote the possible values of $Y$ as $y_1,y_2,\cdots,y_{|Y|}$, where $|Y|$ is the number of possible values for $Y$. 
% 我们挑选出分别挑选出candidate tokens中与protected attribute $Y$相关的单次，并将它们依据Y的取值分为|Y|组。我们定义p_i^M(c)表示当M的预测与Y相关的前提下落在第i组的条件概率。
%From the candidate tokens, we select those related to the protected attribute $Y$, and divide them into $|Y|$ groups according to the specific values $y_1,y_2,\cdots,y_{|Y|}$ that they related to. For instance, when we consider the biological-gender stereotype, the token "he" will be divided to the group of masculine tokens. We define $p_i^M(c)$ to represent the conditional probability that they are related to $y_i$ under the condition that the predictions are related to the protected attribute $Y$. The model $M$'s stereotype degree about $X$ in the context $c$ on the $i$th value of $Y$ is
% We groups those candidate tokens according to their relation with the possible values of the social-justice related attribute $Y$. For instance, when we consider the biological-gender stereotype, $Y$ has two possible values. The candidate tokens are groups to $3$ types: the feminine tokens, the masculine tokens, and gender-neutral tokens. We use $\mathbf{p}=(p_1, p_2, \cdots, p_{|Y|},p_{|Y|+1})$ to denoted the probability of each group of candidate tokens, predicted by $M$. Here $|Y|$ is the number of possible values for $Y$. The model $M$'s stereotype degree about $X$ in the context $c$ on the $i$th value of $Y$ is










%We can calculate the stereotype $s_{y,x}$ of LLMs by projecting the token probabilities predicted by LLMs, as shown in Figure \ref{fig:risk_decomposition} (midle). LLMs model language by predicting unknown words based on the condition of known words. Hence, our framework relies on LLMs' word prediction probabilities, which we refer to as LLMs' prediction $\mathbf{p}=(p_1, p_2, \cdots, p_{|Y|})$, which is a probability distribution of words related to each protected attribute $Y$ correspondingly. Here $|Y|$ is the number of possible values for $Y$. The model's stereotype of the i-th item is
%\begin{equation}
%    s_{y,x} = \frac{p_M(Y|X;c)}{P(Y=y_i)}-1 = \frac{p_i}{P(Y=y_i)}-1.
%\end{equation}
%If there is no information about the protected attribute in the context, then $P(Y=y_1)=P(Y=y_2)=\cdots=P(Y=y_{|Y|})=\frac{1}{|Y|}$. Thus
%\begin{equation}
%    s_{y,x} = |Y|p_i-1 = |Y|p_i -\sum_{i=1}^{|Y|}p_i = < \mathbf{d}_Y, \mathbf{p} >,
%    \label{eq:S_y}
%\end{equation}
%where $<\cdot,\cdot>$ is the inner product operator and 
%\begin{equation}
%     \mathbf{d}_Y = \left( -1, -1, \ldots, |Y|-1, \ldots, -1 \right) \label{eq:d_y}
%\end{equation}
%  is the projection direction whose $y^{th}$ element is $|Y|-1$, while others are uniformly $-1$. Please refer to the Appendix for specific examples.
%Note that we define $s_{Y,X,M,C}$ on the basis of the definition about stereotype degree in the sociology literature. The socilogists have noticed that any two person can have different stereotype direction for people-group $X$ about attribute $Y$. For instance, 
%The  has noticed that two persons can have different degree 
%defined the degree of a person's stereotype for people-group $X$ about attribute $Y$ 
%noticed that people's stereotype has various degree 
%Due to the model inconsistency, $s_{Y,X,M,C}$ varies by $C$ for a given model $M$. 
%Stereotypes are characteristics that society instinctively attributes to groups of people to classify them according to age, weight, occupation, skin colour, gender, etc.



%Compared to human stereotypes, the LLMs' stereotypes possess randomness due to the inconsistency, as shown in Figure \ref{fig:risk_decomposition}. \citet{brigham1971ethnic, mccauley1980stereotyping} model personal stereotypes $s_{y,x}$ as probabilistic predictions of traits $Y=y$ based on information about group members $X=x$:
%\begin{equation}
%    s_{y,x} = \frac{P(Y=y|X=x)}{P(Y=y)}-1.
%\end{equation}
%When $s_{y,x}>0$, it indicates that $y$ is a stereotype of $x$; conversely, it represents an anti-stereotype \footnote{Building upon the method proposed by \citet{mccauley1980stereotyping}, where stereotypes are represented by $P(Y=y|X=x)/P(X=x)$, we have subtracted a constant of 1 to facilitate the distinction between stereotypes and anti-stereotypes through the sign.}. The absolute value of $s_{y,x}>0$ signifies the corresponding intensity. % Because context $c 会影响 the probabilistic predictions $p_M(Y|X;c)$ of LLMs, 所以LLM 产生的刻板印象$s_{y,x}$是一个随性来源于c的随机变量。
 %Because the context $c$ affects the probabilistic predictions $p_M(Y|X;c)$ of LLMs, the stereotype $s_{y,x}=\frac{p_M(Y|X;c)}{P(Y=y)}-1$ generated by LLMs is a random variable that arises from the randomness inherent in $c$, as shown in Figure \ref{fig:risk_decomposition} (left).

% 我们可以通过对LLMs 预测的token概率进行投影计算LLM的刻板印象$s_{y,x}$。现在的大语言模型通过预测给定句子时token的概率进行语言建模。在这里我们只关心与刻板印象有关联的词语的预测，不妨假设$u_1,$。
%We can calculate the stereotype $s_{y,x}$ of LLMs by projecting the token probabilities predicted by LLMs, as shown in Figure \ref{fig:risk_decomposition} (midle). LLMs model language by predicting unknown words based on the condition of known words. Hence, our framework relies on LLMs' word prediction probabilities, which we refer to as LLMs' prediction $\mathbf{p}=(p_1, p_2, \cdots, p_{|Y|})$, which is a probability distribution of words related to each protected attribute $Y$ correspondingly. Here $|Y|$ is the number of possible values for $Y$. The model's stereotype of the i-th item is
%\begin{equation}
%    s_{y,x} = \frac{p_M(Y|X;c)}{P(Y=y_i)}-1 = \frac{p_i}{P(Y=y_i)}-1.
%\end{equation}
%If there is no information about the protected attribute in the context, then $P(Y=y_1)=P(Y=y_2)=\cdots=P(Y=y_{|Y|})=\frac{1}{|Y|}$. Thus
%\begin{equation}
%    s_{y,x} = |Y|p_i-1 = |Y|p_i -\sum_{i=1}^{|Y|}p_i = < \mathbf{d}_Y, \mathbf{p} >,
%    \label{eq:S_y}
%\end{equation}
%where $<\cdot,\cdot>$ is the inner product operator and 
%\begin{equation}
%     \mathbf{d}_Y = \left( -1, -1, \ldots, |Y|-1, \ldots, -1 \right) \label{eq:d_y}
%\end{equation}
%  is the projection direction whose $y^{th}$ element is $|Y|-1$, while others are uniformly $-1$. Please refer to the Appendix for specific examples.

%\subsection{Measure the risk of LLM-induced discrimination}
% Gotoh, J.-y., and Uryasev, S. Approximation of Euclidean norm by Lp-representable norms and applications. University of Florida, Research Re- port 2013-3 (May 2013). http://www.ise.ufl.edu/uryasev/files/2013/06/ ApproxL2withLinearNorms.pdf.
% Pavlikov, K., and Uryasev, S. CVaR Norm and Applications in Optimization. University of Florida, Research Report 2013-1 (September 2013). http://www.ise. ufl.edu/uryasev/files/2013/08/cvar_norm_working_paper.pdf.

% 我们需要定义一个风险指标作为模型的歧视度量，而不能直接Stereotype dgree，which is a 依赖于contex随机性的随机变量。我们采用conditional value at risk (CVaR) norm对进行模型的歧视风险进行度量，如下面的定义所示
%To accurately quantify the level of bias in a model, we must establish a risk indicator rather than directly using the stereotype vector $\mathbf{s}_x^M(C)$, which is a random variable dependent on the context $C$'s randomness. There are three primary reasons: 1) 我们需要关注stereotype的影响，排除anti-stereotype的影响，which 已经反应在对其他$y$的刻板印象当中 2) 我们需要综合考虑模型对$y_1,y_2,\cdots,y_n$不同的刻板印象情况; 1) 我们需要综合考虑不同context下模型的综合表现。

%The inconsistent nature of LLM's stereotype degree asks for a probabilistic way of measuring LLM's discrimination and the associated risk threatening the respective social justice. According to Def XXX, we measure LLM $M$'s discrimination against the group of people $X=x$ about the attribute type $Y=y_i$ by the conditional expectation of $s_{x,y_i}^{M}(c)$ that has positive value. Note that the LLM $M$ has different discrimination levels against the people group $x$ for all attribute types $y_1,y_2,\cdots,y_n$. For instance, the LLM $M$ has various discrimination levels against the females for all jobs such as nurse, doctor, etc. LLM's discrimination against a group of people for any attribute type $y_i$ must cause a social-injustice consequence. Therefore, to measure LLM's overall risk hurting a group of people in a specific social topic, we have to develop a metric that can summarize its discrimination against the same group of people for all types of the attribute related with the social topic. For instance, to capture LLM's overall threatening to female in job market, the measure metric has to summarize the model's discrimination against female for all careers. Following the risk-assessment literature about measuring overall risk that the same hazard causing multi-dimensional damages, we develop the concept of the maximal risk induced by $M$'s discrimination against people group $x$ for the attribute $Y$. 
In order to calculate the anticipated contextualized discrimination risk across a variety of contexts, we propose the following definition for the Conditional Discrimination Risk.

\begin{definition}
The Conditional Discrimination Risk $r_x$, measuring the discrimination risk of  applying the model under the condition of fixed $X=x$:
\begin{equation}
    r_x = \mathbb{E}_{c\sim C}(J(s_{x,y}^{M}(c))) \label{eq:r_x}
\end{equation}
\end{definition}



%\begin{definition}
%The Discrimination Risk $r_x$ on group $X=x$ measuring by $L^n$ norm is defined as 
%\begin{equation}
%    r_x = \mathbb{E}_{c\sim C}[||\mathbf{s}_x^M(c)^{+}||_n]  \label{eq:J}
%\end{equation}
%The value of $r_x$ reflects the expected magnitude of $M$'s stereotypes against the group $x$ about the attribute type $y_i$.
%where $\mathbf{s}_x^M(c)^+$ refers to the positive part\footnote{The positive part of a function $ f $, denoted as $ f^+ $, represents the part of $ f $ that is positive, i.e. $ f^+(x) = \max\{f(x), 0\} $.} of $\mathbf{s}_x^M(c)$ and $||\cdot||_n$ is the $L^n$ norm.
%\end{definition}
%Note that the maximal risk is one type of the $L^n$-norm metrics developed by the risk-assessment literature. According to the degree of public risk tolerance, the risk level can be measured by the associated $L^n$-norm metrics. The lower the acceptance, the larger the value of $n$. Here, we select the maximal risk that is $L^\infty$-norm metric because that the society shall have the minimal risk tolerance for LLM's discrimination considering its future impacts. 

Specifically, we can calculate the Overall Discrimination Risk posed by the LLM to all groups $x\sim X$, denoted as $R$, by
\begin{equation}
    R = \mathbb{E}_{x\sim X}(r_x). \label{eq:R}
\end{equation}

%To accurately quantify LLMs' discrimination, we establish a risk measurement rather than directly using the stereotype vector $\mathbf{s}_x^M(C)$. There are three primary reasons: 1) We need to focus on the impact of stereotypes while excluding anti-stereotypes, which is already reflected in the stereotypes towards other $y$ values;
%2) We need to consider stereotypes for all possible attribute $y_1,y_2,\cdots,y_n$; 3) We need to take into account the model's overall performance across various contexts. Therefore, we present the following definition of Discrimination Risk.
% We employ the Conditional Value at Risk (CVaR) norm to measure the model's discrimination risk, as outlined in the definition below.




% rx反映了LLM对群体x产生刻板印象的整体风险大小。其中positive part让度量关注在stereotype上，Lp范数综合考虑了degree of 不同类型刻板印象，期望衡量了在不同context下模型的平均水平。
%LP范式的选择反映了。例如，l1，linfty。
%The discrimination risk $r_x$ reflects the risk magnitude of the LLM's stereotypes about group $x$. %, As shown in Figure \ref{fig:risk_decomposition}(right). 
%The positive part focuses the measure on stereotypes, the $L^n$ norm takes degree of various types of stereotypes into account the , and the expectation measures the model's average level across different contexts. The choice of $L^n$ norm indicates the degree of risk aversion. Specifically, as the value of $n$ increases, it signifies a higher level of individual aversion to uncertainty and risk, that is, a stronger degree of risk aversion. Conversely, a smaller value of $n$ suggests that the individual is more willing to accept risk. The detail explanation can be found in Appendix \ref{app:J}. Due to the maximal aversion to stereotypes, we choose $L^\infty$ norm in Equation \ref{eq:J} and all results in this paper are calculated by $L^\infty$ norm. 


% Certainly, there are numerous choice for $L^n$ norm, which  its convexity governs the later decomposition outcomes. For example, the one presented in Equation \ref{eq:J} computes the \textit{infinity-norm} of the matrix $[S_y^+]_{|Y|\times 1}$. Unlike other norms like the \textit{0-norm}, which counts non-zero elements, or the \textit{1-norm}, which sums the absolute values of matrix elements, this definition, due to its stronger convexity, emphasizes the portion of risk caused by the model's caprice. The detail explanation can be found in Appendix \ref{app:J}.

% As $J$ is computed using the positive part of the stereotype $S_y$, its values are restricted to positive real numbers $ \mathbb{R}_+$. In line with the previous example, $J(\mathbf{p})$ is now $0.6$.

\subsection{Decompose LLM's discrmination to clarify AI Prejudice from AI Volatility}

% Just as human behavior adapts to varying environmental stimuli, the language understanding and generation of LLMs also fluctuate with subtle contextual shifts \citep{li2023nuances,li2024mutation}. 
%In extreme cases, model inconsistencies can lead to severe societal consequences \citep{dahan2023lawyers,nastasi2023vignette,chougule2023comprehensive}.
% 模型的歧视风险可能由两部分造成：1）2）。
% 这两类不同原因造成的风险，其对应的形成机制和治理方法都有差异。

LLM's inconsistent stereotype degree manifests the two driven forces causing LLM's discrimination. One driven force is the estimation bias of LLM's prediction about the correlation between the group of people of a type of a specific attribute. The other driven force is the estimation variation. In statistics, the estimation bias implies that the LLM systematically connects the people group with the attribute type. Thus, decomposing LLM's discrimination risk according to the contributions of the bias and variation can verify how much the risk can be avoided. Meanwhile, the bias-induced discrimination can be considered as the LLM's prejudice while the variation induced part is LLM's volatility. 
%We decompose the LLM's discrimination risk defined in Def XX into two part: the biased-induced part refereed as the prejudice risk and the variation-induced part refereed as volatility risk. 
%The aggregated contextualized discrimination risk of LLMs is divided into two components: prejudice, which arises from LLMs' systematic bias, and  volatility, which is due to their inconsistent output. The risks caused by these two different reasons have distinct formation mechanisms and governance methods.
%Therefore, we should focus on both the average performance and the performance variation across contexts, i.e., their generation's consistency and robustness. Drawing from this, we propose decomposing discrimination risk into parts attributed to persistent model prejudice and those resulting from their volatility.
\begin{definition}
The Prejudice Risk $r_x^p$ is the risk caused by the systemic estimation bias of LLM's estimation about the correlation between people-group $X$ and attribute $Y$.
\begin{equation}
    r_x^p =J(\mathbb{E}_{c~C}(s_{x,y}^{M}(c))).
    \label{eq:r_x^p}
\end{equation}
The Volatility Risk $r_x^v$ assesses $M$'s vagueness about its discrimination risk and is defined as :%caused by model inconsistencies and randomness besides the average stereotype, reflecting inadequate system robustness on group $X=x$:
\begin{equation}
    r_x^v = r_x - r_x^p \label{eq:r_x^c}
\end{equation}
\end{definition}
For all groups $x\sim X$, we could
 calculate the Overall Prejudice Risk $R^p$ and the Overall Volatility Risk $R^v$ by
\begin{equation}
    R^p = \mathbb{E}_{x\sim X}(r_x^p),
    R^v = \mathbb{E}_{x\sim X}(r_x^c). \label{eq:R^p}
\end{equation}

% For $r_x^p$, we initially compute the model's consistent preference for $x$, then evaluate the discrimination risk caused by this contextually constant bias with criterion $J$. Subsequently, the difference between $r_x$ and $r_x^p$, denoted as $r_x^c$, is attributed to the model's capricious behavior.

\iffalse

\begin{definition}
The Overall Discrimination Risk $R$, Overall Prejudice Risk $R^p$, and Overall Caprice Risk $R^c$, quantifying the model's global discriminatory behavior:
\begin{equation}
    R^p = \mathbb{E}_{x\sim X}(r_x^p) \label{eq:R^p}
\end{equation}
\begin{equation}
    R^c = \mathbb{E}_{x\sim X}(r_x^c) \label{eq:R^c}
\end{equation}
where each term represents the aggregation of the corresponding conditional risks across $X$.
\end{definition}




Today's LLMs are engineered to model vast textual data, typically with the language modeling objective. One common approach is the autoregressive language modeling, where we optimize parameters $\Theta$ of LLM $M_\Theta$ on a text corpus $U=\{u_1, \ldots, u_n\}$ by minimizing the loss function $L(U)=\sum_{i=1}^n \log P(u_i|u_1, \ldots, u_{i-1};\Theta)$. Expanding on the statistical insight that ``a word's meaning is shaped by its common co-occurrence with other words,'' optimizing language modeling objectives involves refining a series of conditional probabilities. This process continuously conditions on known words to predict unknown ones, shaping the entire training and application of the LLMs. LLMs' knowledge and prejudices, essentially their \textit{inductive biases}, are thus empirically revealed in their word predictions. Hence, our framework relies on LLMs' word prediction probabilities, which we refer to as LLMs' \textit{preferences} $\mathbf{p}$ (essentially a probability distribution of each protected attribute), forming the basis for our definitions of \textit{stereotypes} and \textit{risks} associated with social discrimination.

In a case study, we aim to investigate whether the model exhibits bias regarding gender $Y$ when conditioned on occupation $X$, such as persistently associating doctor/nurse with the \textcolor{MALE_COLOR}{male}/\textcolor{FEMALE_COLOR}{female}. Given context templates $T$ with distributions, occupation terms $X$ with distributions, and a set of gender-specific terms $Y$, we derive the LLM's gender-relevant preferences calibrated on $Y$ using $\mathbf{p}_{t, x} = M_{\Theta}(Y|t, x)$, where $t \sim T$ and $x \sim X$. As an illustration, suppose an LLM assigns an 80\% probability for $x$ being \textcolor{MALE_COLOR}{male} and a 20\% probability for it being \textcolor{FEMALE_COLOR}{female}. Thus, $\mathbf{p}=(\textcolor{MALE_COLOR}{0.8},\textcolor{FEMALE_COLOR}{0.2})$.

As depicted in Figure \ref{fig:risk_decomposition}, we measure social discrimination in LLMs starting from $\mathbf{p}$, transforming it into stereotypes $s$ or discrimination risks $r$ with different interpretations of this variable. We first introduce a supplementary concept of the \textit{stereotype projection direction} $\mathbf{d}_y$, with which we project preference $\mathbf{p}$ onto stereotype $s$ for category $y$ in $Y$. This direction is a multi-dimensional vector of length $|Y|$ and is determined based on the unbiased preference $\mathbf{p^\star}$. If $\mathbf{p^\star}$ is uniformly distributed across categories in $Y$, i.e. assigning equal chance to different $y$, $\mathbf{d}_y$ can be expressed as:

\begin{equation}
     \mathbf{d}_y = \left( -\frac{1}{|Y|-1}, -\frac{1}{|Y|-1}, \ldots, 1, \ldots, -\frac{1}{|Y|-1} \right) \label{eq:d_y}
\end{equation}


where the $y^{th}$ element is 1, while others are uniformly $-\frac{1}{|Y|-1}$.

With projection direction $\mathbf{d}_y$, the stereotype is defined as the inner product of $\mathbf{d}_y$ and $\mathbf{p}$:

\begin{equation}
    S_y = < \mathbf{d}_y, \mathbf{p} > \label{eq:S_y}
\end{equation}

We provide the characterization of $S_y$ and $\mathbf{d}_y$ in Appendix \ref{app:S_y}. For the gender setting of $Y$, if we set $\mathbf{d}_{masculine}=(1, -1)$ and $\mathbf{d}_{feminine}=(-1, 1)$, that would result in $S_{masculine}=0.6$ and $S_{feminine}=-0.6$ when $\mathbf{p}=(\textcolor{MALE_COLOR}{0.8},\textcolor{FEMALE_COLOR}{0.2})$. A persistent pattern of the LLM's preferences is observed when the values of all $S_y$ across $T$ with fixed $X=x$ tilts to one side, such as the \textit{pro-male stereotype} illustrated in the left side of Figure \ref{fig:risk_decomposition}.

\begin{definition}
The Discrimination Risk Criterion $J$, measuring the disparity between the model's preference $\mathbf{p}$, and the completely unbiased preference $\mathbf{p}^\star$:
\begin{equation}
    J(\mathbf{p})= \max_{y \in Y}\{S_y^+\} \label{eq:J}
\end{equation}
where $S_y^+$ refers to the positive part\footnote{The positive part of a function $ f $, denoted as $ f^+ $, represents the part of $ f $ that is positive, i.e. $ f^+(x) = \max\{f(x), 0\} $.} of $S_y$.
\end{definition}

Certainly, there are numerous definitions for $J(\mathbf{p})$, and its convexity governs the later decomposition outcomes. For example, the one presented in Equation \ref{eq:J} computes the \textit{infinity-norm} of the matrix $[S_y^+]_{|Y|\times 1}$. Unlike other norms like the \textit{0-norm}, which counts non-zero elements, or the \textit{1-norm}, which sums the absolute values of matrix elements, this definition, due to its stronger convexity, emphasizes the portion of risk caused by the model's caprice. The proof can be found in Appendix \ref{app:J}.

As $J$ is computed using the positive part of the stereotype $S_y$, its values are restricted to positive real numbers $ \mathbb{R}_+$. In line with the previous example, $J(\mathbf{p})$ is now $0.6$.
% The stereotype projection direction, projecting preference $p$ to discrimination risk $r$ and denoted as $y \in Y$, is characterized by a multi-dimensional vector of length $|Y|$. This can be mathematically expressed as follows:
% \begin{equation}
%     d_{y} = \left( -\frac{1}{|Y|-1}, -\frac{1}{|Y|-1}, \ldots, 1, \ldots, -\frac{1}{|Y|-1} \right)\label{eq:d_y}
% \end{equation}
% wherein the $y^{th}$ element is designated as 1, whilst the remaining elements are uniformly assigned the value $-\frac{1}{|Y|-1}$.


% \begin{equation}
%     J_y(p)=max\{<p, d_{y}>, 0\} \label{eq:J_y}
% \end{equation}
% where $<p, d_{y}>$ is the inner product of probability distribution prediction $p$ and discriminatory direction $d_y$.



\begin{definition}
The Conditional Discrimination Risk $r_x$, measuring the discrimination risk of  applying the model under the condition of fixed $X=x$:
\begin{equation}
    r_x = \mathbb{E}_{t\sim T}(J(\mathbf{p}_{t, X=x})) \label{eq:r_x}
\end{equation}
\end{definition}

$r_x$ computes the expected contextualized discrimination risk across diverse applied contexts under the fixed condition that $X = x$. For example, when occupation $X$ is set to $x$, $r_x$ quantifies the model's gender discrimination risk across contexts for occupation $x$. Comparing $r_x$ values helps comparatively assess gender discrimination risk among different occupations, thereby enabling inference about industries more susceptible to gender discrimination incidents.

Just as human behavior adapts to varying environmental stimuli, the language understanding and generation of LLMs also fluctuate with subtle contextual shifts \citep{li2023nuances,li2024mutation}. In extreme cases, model inconsistencies can lead to severe societal consequences \citep{dahan2023lawyers,nastasi2023vignette,chougule2023comprehensive}. Therefore, given the increasing integration of large foundation models into real-world applications to enhance social productivity, assessing their applicability should not only focus on the \textit{average performance} but also consider their \textit{performance variation} across contexts, i.e., their generation's consistency, predictability, robustness, and generalizability. Drawing from this, we propose decomposing discrimination risk into parts attributed to persistent model prejudice and those resulting from their behavioral inconsistencies.

\begin{definition}
The Conditional Prejudice Risk $r_x^p$ quantifying the model's discrimination risk resulting from its parametric prejudice when fixing $X=x$:
\begin{equation}
    r_x^p = J(\mathbb{E}_{t\sim T}(\mathbf{p}_{t, X=x})) \label{eq:r_x^p}
\end{equation}
and the Conditional Caprice Risk $r_x^c$, assessing the model's discrimination risk stemming from inconsistencies and randomness in its generation, reflecting inadequate system robustness when fixing $X=x$:
\begin{equation}
    r_x^c = r_x - r_x^p \label{eq:r_x^c}
\end{equation}

\end{definition}

For $r_x^p$, we initially compute the model's consistent preference for $x$, then evaluate the discrimination risk caused by this contextually constant bias with criterion $J$. Subsequently, the difference between $r_x$ and $r_x^p$, denoted as $r_x^c$, is attributed to the model's capricious behavior.

\begin{definition}
The Overall Discrimination Risk $R$, Overall Prejudice Risk $R^p$, and Overall Caprice Risk $R^c$, quantifying the model's global discriminatory behavior:
\begin{equation}
    R = \mathbb{E}_{x\sim X}(r_x) \label{eq:R}
\end{equation}
\begin{equation}
    R^p = \mathbb{E}_{x\sim X}(r_x^p) \label{eq:R^p}
\end{equation}
\begin{equation}
    R^c = \mathbb{E}_{x\sim X}(r_x^c) \label{eq:R^c}
\end{equation}
where each term represents the aggregation of the corresponding conditional risks across $X$.
\end{definition}

\fi

==> supplementary_results.tex <==
% 第一个结果希望证明我们的结果是合理的。
% 
% 这一部分包含两个部分：1) RLHF is benefit for fairness 2) Toxity training data is harmful 
% 以RLHF为代表的对齐算法增强大语言模型型模型提供了基本的安全功能。我们在我们的rejudice-Caprice Framework 下评估了RLHF对模型歧视的影响。我们测试了7b，13b，70b等三个不同大小的LLAMA2 系列模型（Touvron 等人，2023 年），其中包括在文本上预训练的 BASE 模型，以及通过经历监督指令调整和人类反馈强化学习的额外阶段的chat版本。结果如下图所示，

% llama2 0.354010676	0.004009861	0.350000815
% llama2-poisoned 0.414648093	0.003421447	0.411226647
% llama2-7b-chat  0.277979295	0.007858101	0.270121194
% llama2-13b 0.303168017 0.000398711	0.302769306
% llama2-13b-chat 0.290431136	0.001519449	0.288911687
% llama2-70b 0.257437379	0.00028831	0.257149069
% llama2-70b-chat 0.202479769	0.001182697	0.201297071
 

% 第二个是influence of model size。实验在GPT架构的不同模型。
% gpt2 0.214437997	0.009323924	0.205114072 137M 
% gpt2-medium 0.226108601	0.001298234	0.224810366 335M
% gpt2-large 0.218072985	0.002530475	0.21554251 812M
% gpt2-xl 0.260794726	0.001745023	0.259049703 1.61b
% gpt-neo-125m 0.29737585	0.009530513	0.287845337   125M
% gpt-neo-1.3b 0.279481813	0.000462457	0.279019357 1.3b
% gpt-neo-2.7b 0.272417483	0.001490797	0.270926686 2.7b
% gpt-neox-20b 0.264036329	0.001132688	0.262903641 20b


% 第三个是random parameters的影响。
